Linguistically-Informed Neural Architectures for Lexical, Syntactic and Semantic Tasks in Sanskrit

The primary focus of this thesis is to make Sanskrit manuscripts more accessible to the end-users through natural language technologies. The morphological richness, compounding, free word orderliness, and low-resource nature of Sanskrit pose significant challenges for developing deep learning solutions. We identify four fundamental tasks, which are crucial for developing a robust NLP technology for Sanskrit: word segmentation, dependency parsing, compound type identification, and poetry analysis. The first task, Sanskrit Word Segmentation (SWS), is a fundamental text processing task for any other downstream applications. However, it is challenging due to the sandhi phenomenon that modifies characters at word boundaries. Similarly, the existing dependency parsing approaches struggle with morphologically rich and low-resource languages like Sanskrit. Compound type identification is also challenging for Sanskrit due to the context-sensitive semantic relation between components. All these challenges result in sub-optimal performance in NLP applications like question answering and machine translation. Finally, Sanskrit poetry has not been extensively studied in computational linguistics. While addressing these challenges, this thesis makes various contributions: (1) The thesis proposes linguistically-informed neural architectures for these tasks. (2) We showcase the interpretability and multilingual extension of the proposed systems. (3) Our proposed systems report state-of-the-art performance. (4) Finally, we present a neural toolkit named SanskritShala, a web-based application that provides real-time analysis of input for various NLP tasks. Overall, this thesis contributes to making Sanskrit manuscripts more accessible by developing robust NLP technology and releasing various resources, datasets, and web-based toolkit.

==> Chapters/Chapter7.tex <==
% Chapter Template

\chapter{SanskritShala: A Neural Sanskrit NLP Toolkit with Web-Based Interface for Pedagogical and Annotation Purposes}

\label{Chapter7}

\lhead{Chapter 7. \emph{SanskritShala: A Neural Sanskrit NLP Toolkit}}

We present  a  neural  Sanskrit  Natural Language Processing (NLP)  toolkit named SanskritShala\footnote{It means `a school of Sanskrit'.} to facilitate computational linguistic analyses for several tasks such as word segmentation, morphological tagging, dependency parsing, and compound type identification. Our systems currently report state-of-the-art performance on available benchmark datasets for all tasks. SanskritShala is deployed as a web-based application, which allows a user to get real-time analysis for the given input. It is built with easy-to-use interactive data annotation features that allow annotators to correct the system predictions when it makes mistakes. We publicly release the source codes of the 4 modules included in the toolkit, 7 word embedding models that have been trained on publicly available Sanskrit corpora and multiple annotated datasets such as word similarity, relatedness, categorization, analogy prediction to assess intrinsic properties of word embeddings.  So far as we know, this is the first neural-based Sanskrit NLP toolkit that has a web-based interface and a number of NLP modules. We are sure that the people who are willing to work with Sanskrit will find it useful for pedagogical and annotative purposes. SanskritShala is available at: \url{https://cnerg.iitkgp.ac.in/sanskritshala}. The demo video of our platform can be accessed at: \url{https://youtu.be/x0X31Y9k0mw4}.

\section{Motivation}
Sanskrit is a culture-bearing and knowledge-preserving language of ancient India. Digitization has come a long way, making it easy for people to access ancient Sanskrit manuscripts \cite{goyal-etal-2012-distributed,adiga-etal-2021-automatic}. 
However, we find that the utility of these digitized manuscripts is limited due to the  user's lack of language expertise and various linguistic phenomena exhibited by the language.
% Each ancient Indian discipline has its own technique for interpreting and teaching Sanskrit literature. 
% To understand the original Sanskrit text, one must be proficient in Sanskrit grammar, which is time-consuming and tiresome. 
% People who lack grammatical background can not comprehend the original Sanskrit texts. On the other hand, the secondary sources like available Sanskrit commentaries are also not useful for individuals due to lack of language expertise. 
This motivates us to investigate how we can utilize natural language technologies to make Sanskrit texts more accessible.

The aim of this research is to create neural-based Sanskrit NLP systems that are accessible through a user-friendly web interface. The Sanskrit language presents a range of challenges for building deep learning solutions, such as the \textit{sandhi} phenomenon, a rich morphology, frequent compounding, flexible word order, and limited resources \cite{translist,Graph-Based,sandhan-etal-2021-little,sandhan-etal-2019-revisiting}. To overcome these challenges, 4 preliminary tasks were identified as essential for processing Sanskrit texts: word segmentation, morphological tagging, dependency parsing, and compound type identification. The word segmentation task is complicated by the \textit{sandhi} phenomenon, which transforms the word boundaries \cite{translist}. The lack of robust morphological analyzers makes it challenging to extract morphological information, which is crucial for dependency parsing. Similarly, dependency information is essential for several downstream tasks such as word order linearisation \cite{krishna-etal-2019-poetry} which helps to decode possible interpretation of the poetic composition. Additionally, the ubiquitous nature of compounding in Sanskrit is difficult due to the implicitly encoded semantic relationship between its constituents \cite{sandhan-etal-2022-novel}. 
% This work focuses on the development of neural-based Sanskrit NLP systems  that are integrated with user-friendly web-based interface.
%  The \textit{sandhi} phenomenon, morphological richness, compounding, relatively free word orderliness and low resource nature pose challenges for building deep learning solutions for Sanskrit \cite{translist,Graph-Based,sandhan-etal-2021-little,sandhan-etal-2019-revisiting}.
%  We identify 4 preliminary tasks, which are essential for processing Sanskrit texts: (1) word segmentation, (2) morphological tagging, (3) dependency parsing and (4) compound type identification\footnote{It is a multi-class classification problem where task is to identify implicitly encoded semantic relation between the two components of a binary compound.}. Although word segmentation is the most basic step in text processing, it is not trivial for Sanskrit due to the \textit{sandhi} phenomenon, which transforms phonemes at the word boundaries \cite{translist}. 
% Morphological information is essential for dependency parsing, but the lack of robust analyzers makes it difficult to extract this information for Sanskrit \cite{sandhan-etal-2021-little}. Similarly, dependency information is essential for several downstream tasks such as word order linearisation \cite{krishna-etal-2019-poetry} which helps to decode possible interpretation of the poetic composition.
% Lastly, compounding is ubiquitous in Sanskrit, which is difficult due to the implicitly encrypted context-sensitive semantic relationship between the compound's constituents \cite{sandhan-etal-2022-novel}.  As a result, the Sanskrit NLP applications such as machine translation and question answering display sub-optimal performance when they come across
% compounds.  
These 4 tasks can be viewed as a preliminary requirement for developing robust NLP technology for Sanskrit.  
Thus, we develop novel neural-based linguistically informed architectures for all 4 tasks, reporting state-of-the-art performance on Sanskrit benchmark datasets \cite{sandhan-etal-2022-novel,translist,sandhan_systematic}. 
 We also illustrate the efficacy of our language agnostic proposed systems in multiple low-resource languages. 

In this work, we introduce  a  neural  Sanskrit  NLP toolkit named SanskritShala\footnote{Roughly, it can be translated as `a school of Sanskrit'.} to assist computational linguistic analyses involving multiple tasks such as word segmentation, morphological tagging, dependency parsing, and compound type identification.
SanskritShala is also deployed as a web application that enables users to input text and gain real-time linguistic analysis from our pretrained systems. It is also equipped with user-friendly interactive data annotation capabilities that allow annotators to rectify the system when it makes errors. It provides the following benefits: (1) A user with no prior experience with deep learning can utilise it for educational purposes. (2) It can function as a semi-supervised annotation tool that requires human oversight for erroneous corrections.   
We publicly release the source code of the 4 modules included in the toolkit, 7 word embedding models that have been trained on publicly available Sanskrit corpora and multiple annotated datasets such as word similarity, relatedness, categorization, analogy prediction to measure the word embeddings' quality.
 To the best of our knowledge, this is the first neural-based Sanskrit NLP toolkit that contains a variety of NLP modules integrated with a web-based interface.
% Inspired from the available Sanskrit resources such as Sanskrit Heritage Reader \cite{} and Sa\d{m}s\={a}dhani \cite{}, we deploy our pretrained

Summarily, our key contributions are as follows:
\begin{itemize}
    \item We introduce the first neural Sanskrit NLP toolkit to facilitate automatic linguistic analyses for 4  downstream tasks (\S \ref{neural_toolkit}).
    \item We release 7 pretrained Sanskrit embeddings and suit of 4 intrinsic evaluation datasets to measure the word embeddings' quality.
    \item We integrate SanskritShala with a user-friendly web-based interface which is helpful for pedagogical purposes and in developing annotated datasets (\S \ref{webinterface}).
    \item We publicly release codebase and datasets of all the modules of SanskritShala which currently mark the state-of-the-art results.\footnote{\url{https://github.com/Jivnesh/SanskritShala}}
\end{itemize}



\begin{figure*}[!tbh]
    \centering
    % \subfigure[]{\includegraphics[width=0.45\textwidth]{images/ssAAAI-SHR.pdf}\label{fig:SHR2lattice}} 
    \subfigure[]{\includegraphics[width=0.45\textwidth]{images/ssAAAI-model.pdf}\label{fig:flat_architecture_ACL}}
    \subfigure[]
    {\includegraphics[width=0.45\textwidth]{images/LemmaTag.pdf}\label{fig:LemmaTag_ACL}}
    \subfigure[]
    {\includegraphics[width=0.45\textwidth]{images/ssTallip_LCM.pdf}\label{fig:dep_architecture_ACL}}
    \subfigure[]
    {\includegraphics[width=0.45\textwidth]{images/ssCOLING20-Model.pdf}\label{fig:sacti_architecture_ACL}}
    \caption{(a) Toy illustration of the TransLIST system.``{\sl d\={a}sobhava}''. Translation: ``Become a servant.'' (b) LemmaTag architecture in which multi-task learning formulation is leveraged to predict morphological tags and lemmas by employing bidirectional RNNs with character-level and word-level representations. (c) Proposed ensembled architecture for dependency parsing   (d) Toy example illustrating the context-sensitive multi-task learning system: ``{\sl aham p\={\i}ta-ambaram dhar\={a}mi}'' (Translation: ``I wear a yellow cloth'') where `{\sl p\={\i}ta-ambaram}' is a compound having \textit{Tatpuru\d{s}a} semantic class according to the context presented.}
    \label{figure:complete_TransLIST}
\end{figure*}



% \section{About Sanskrit}
\section{A Neural NLP Sanskrit Toolkit}
In this section, we describe SanskritShala, which is a neural Sanskrit NLP toolkit designed to aid computational linguistic analysis including various tasks, such as word segmentation, morphological tagging, dependency parsing, and compound type identification. It is also available as a web application that allows users to input text and obtain real-time linguistic analysis from our pretrained algorithms.
We elucidate SanskritShala by first elaborating on
its key modules.
\label{neural_toolkit}
\noindent\textbf{Word Tokenizer:}
Earlier \textit{lexicon-driven} systems for Sanskrit word segmentation (SWS) rely on Sanskrit Heritage Reader \cite[SHR]{goyaldesign16}, a rule-based system, to obtain the exhaustive solution space for segmentation, followed by diverse approaches to find the most valid solution. However, these systems are rendered moot while stumbling out-of-vocabulary words. Later, \textit{data-driven} systems for SWS are built using the most recent techniques in deep learning, but can not utilize the available candidate solution space.  To overcome the drawbacks of both lines of modelling, we build a \textbf{Tran}sformer-based \textbf{L}inguistically-\textbf{I}nformed \textbf{S}anskrit \textbf{T}okenizer (TransLIST) \cite{translist} containing (1) a component that encodes the character-level and word-level potential candidate solutions, which tackles \textit{sandhi} scenario typical to SWS and is compatible with partially available candidate solution space, (2) a novel soft-masked attention for prioritizing selected set of candidates and (3) a novel path ranking module to correct the mispredictions. 
Figure \ref{fig:flat_architecture_ACL}  illustrates the TransLIST architecture, where the candidate solutions obtained from SHR are used as auxiliary information. 
In terms of the perfect match (PM) evaluation metric, TransLIST surpasses the existing state-of-the-art \cite{hellwig-nehrdich-2018-sanskrit}  by 7.2 absolute points.
\noindent\textbf{Morphological Tagger:}
Sanskrit is a morphologically-rich fusional Indian language with 40,000 possible labels for inflectional morphology \cite{krishna-etal-2020-graph,gupta-etal-2020-evaluating}, where homonymy and syncretism are predominant \cite{krishna-etal-2018-free}. We train a neural-based architecture \cite[LemmaTag]{kondratyuk-etal-2018-lemmatag} on Sanskrit dataset \cite{hackathon}. Figure \ref{fig:LemmaTag_ACL} illustrates the system architecture in which multi-task learning formulation is leveraged to predict morphological tags and lemmas by employing bidirectional RNNs with character-level and word-level representations. We find that both tasks help by sharing the encoder, predicting label subcategories, and feeding the tagger output as input to the lemmatizer \cite{kondratyuk-etal-2018-lemmatag}.
% Additionally, we augment constraints generated by rule-based system SHR during inference by restricting the system to predict from the candidates suggested the rule-based system SHR. 
Currently, our system trained on the Sanskrit dataset stands first on the Hackathon dataset \cite{hackathon} leaderboard. 
\noindent\textbf{Dependency Parser:}
We focus on low-resource Sanskrit dependency parsing. Numerous strategies are tailored to improve task-specific performance in low-resource scenarios.
 Although these strategies are well-known to the NLP community, it is not obvious to choose the best-performing ensemble of these methods for a low-resource language of interest, and not much effort has been given to gauging the usefulness of these methods. We investigate 5 low-resource strategies in our ensembled Sanskrit parser \cite{sandhan_systematic}: data augmentation, multi-task learning, sequential transfer learning, pretraining, cross/mono-lingual and self-training.
Figure \ref{fig:dep_architecture_ACL} shows our ensembled system, which supersedes the current state-of-the-art \cite{krishna-etal-2020-keep} for Sanskrit by 1.2 points absolute gain (Unlabelled Attached Score) and shows on par performance in terms of Labelled Attached Score. Our extensive multi-lingual experimentation on a variety of low-resource languages demonstrates significant improvements for languages that are not covered by pretrained language models.
\noindent\textbf{Sanskrit Compound Type Identifier:}
% Compounding is omnipresent in Sanskrit. It helps achieve brevity in communicating ideas while simultaneously enhancing the lexical and structural appearance of the language.
SaCTI is a multi-class classification task that identifies semantic relationships between the components of a compound. Prior methods only used the lexical information from the constituents and didn't take into account the most crucial syntactic and contextual information for SaCTI. However, the SaCTI task is difficult mainly due to the implicitly encrypted context-dependent semantic relationship between the compound's constituents. 
Thus, we introduce a novel multi-task learning approach \cite{sandhan-etal-2022-novel} (Figure \ref{fig:sacti_architecture_ACL}) which includes contextual information and enhances the complementary syntactic information employing morphological parsing and dependency parsing as two auxiliary tasks. SaCTI outperforms the state-of-the-art by  $7.7$ points (F1-score) absolute gain on the benchmark datasets. 
% Additionally, our multi-lingual investigations confirm the effectiveness of the proposed apporach in English and Marathi languages.
\begin{figure*}[!tbh]
    \centering
    \includegraphics[width=0.9\textwidth]{images/sanskritshala.png}
    \caption{The web interface of the SanskritShala. 
    % The user can pick any standalone task from the homepage or initiate a pipeline starting from the word segmentation task and then morphological tagging and dependency parsing.
    At the bottom right, a rule-based chatbot is added to navigate users on the platform to give users a user-friendly experience.}
    \label{figure:sanskritshala}
\end{figure*}
\begin{figure*}[!tbh]
    \centering
       \subfigure[]{\includegraphics[width=0.45\textwidth]{images/shr.png}\label{fig:shr++}} 
    \subfigure[]{\includegraphics[width=0.45\textwidth]{images/morph.png}\label{fig:morph_tagger}}
    \caption{(a) The candidate solution space generated by SHR for the word segmentation task and the predicted solution by our pretrained model is recommended for the sequence ‘\textit{prabh\={u}tanaran\={a}gena balenopavive\'sa ha}’ using a yellow highlight. We expect a user to select a solution considering the recommendations shown by our system. The figure shows the stage at which the first two segments are selected manually. (b) Morphological Tagger: For each word, we show possible morphological analyses suggested by SHR as well as our system prediction in green if it falls in SHR's candidate space, otherwise in orange. Note that we prefer to use different examples in (a) and (b) for illustrating one of the features of a morphological tagger: If model prediction lies outside of SHR space, then it is highlighted with orange.}
    \label{figure:SHR}
\end{figure*}
\begin{figure*}[!tbh]
    \centering
      \subfigure[]{\includegraphics[width=0.45\textwidth]{images/dp.png}\label{fig:dep_parser}}
       \subfigure[]{\includegraphics[width=0.45\textwidth]{images/sacti.png}\label{fig:sacti}} 
  
\caption{ (a) Dependency parser: Interactive module for the dependency parsing task which directly loads predicted dependency trees from our pretrain model and allows user to correct mispredictions using our interactive interface. (b) Illustration of compound identifier}
    \label{figure:pipeline}
\end{figure*}
\section{Web-based Interface of SanskritShala}
\label{webinterface}
Figure \ref{figure:sanskritshala} shows our SanskritShala toolkit that offers interactive web-based predictions for various NLP tasks. The toolkit is built using React framework, which makes it user-friendly and easy to use. One of the tasks it handles is the word segmentation task, which is built on top of the web-based application called SHR++. The SHR++ demonstration is depicted in Figure \ref{fig:shr++}. The user inputs a Sanskrit string, which is then sent in real-time to SHR for potential word splits. The system prediction is then obtained from the pretrained word tokenizer. The human annotator is presented with the candidate solution space, with the system prediction highlighted in yellow.
The toolkit also features a flask-based application for morphological tagging, which takes user input and scrapes possible morphological tags for each word using SHR. As shown in Figure \ref{fig:morph_tagger}, the predictions of the pretrained morphological tagger are displayed in green or orange, depending on whether they are present in the candidate solution of SHR or not. The user can also add a new tag if the actual tag is missing in the SHR solution space or the system's prediction.
For the dependency parsing module, we have built a react-based front-end. The user input is passed to the pretrained model to generate a dependency structure. As illustrated in Figure \ref{fig:dep_parser}, the front-end automatically loads the predicted dependency tree and allows the user to make corrections if there are any mispredictions. Additionally, Figure \ref{fig:sacti} shows a flask-based application for the compound type identifier, where users can give input to the system through its web interface. The final annotations can be downloaded after each individual module. We plan to maintain the progress of Sanskrit NLP and offer an overview of available datasets and existing state-of-the-art via the leaderboard for various tasks.
% SanskritShala is a Sanskrit NLP toolkit that lets users get predictions for different tasks through an interactive web-based user interface built using React framework. For the word segmentation task, we build on top of the existing web-based application released by \newcite[SHR++]{krishna-etal-2020-shr}.
% Figure \ref{figure:SHR} depicts the SHR++ demonstration with a toy example for the word segmentation task. It provides a web interface that lets the user input a Sanskrit string (word, phrase or sentence). The user input is sent in real-time to SHR to enumerate potential word splits and also to our pretrained word tokenizer for obtaining system predictions.  Figure \ref{figure:SHR} depicts the human annotator being presented with the exhaustive candidate solution space and the system prediction highlighted with yellow. We expect the annotator to recognize/verify the proper segmented word forms and then proceed with the morpho-syntactic analysis of the chosen word forms. Next, we develope a flask-based application for morphological tagging. It takes user input and scrapes possible morphological tags for each word using SHR. As shown in the Figure \ref{fig:morph_tagger},  our pretrained morphological tagger's predictions are shown in green if they fall in candidate solution of SHR otherwise in orange. We expect annotator to verify/modify the predictions. We also allow user to add a new tag if actual tag is missing in SHR solution space including our system's prediction. Thirdly, we build a react-based front-end for the dependency parsing module, as shown in the Figure ~\ref{fig:dep_parser}. User input is passed to our pretrained model to generate a dependency structure. Our front-end automatically loads a predicted dependency tree and allows user to correct if any mispredictions. Finally, we also have flask-based application for compound type identifier, where user can give input to our system via its web interface. We also give option to download the final annotations after each individual module. Apart from this, we are also planning to maintain Sanskrit NLP progress.\footnote{\url{http://cnerg.iitkgp.ac.in/sanskritshala/resources}} It will facilitate users to get an overview of available datasets and existing state-of-the-art via the leaderboard for the tasks.

\noindent\textbf{Interactive Chatbot:}
SanskritShala-bot is a rule-based chatbot that makes it easy to automate simple and repetitive user requests, like answering frequently asked questions and directing users to relevant resources. It is also easier to set up and maintain than AI-powered chatbots, which are more complicated, which makes them a good choice for us with limited resources. SanskritShala-bot is especially useful for helping many users quickly and effectively. It helps familiarize users with a platform by providing them with information and guidance on how to use it. It can answer questions about the platform's features, help users find their way around it, and explain step-by-step how to do certain tasks. This can make it easier for users to get started and  leading to a better experience. 


%  \begin{figure*}[!h]
% \centering
% % \includegraphics[width=0.3\textwidth]{images/Annotations.jpeg}
% \subfigure[]{\includegraphics[width=1.5in,height=2in]{images/Annotations.jpeg}}\qquad \qquad
% \subfigure[]{\includegraphics[height=1.5in,height=2in]{images/Interface_admin.jpeg}}
% \caption{Illustration of our web-based mobile friendly (a) annotation interface, where the task is to select the correct option from multiple-choices for the given compound with the context. (b) Administrative interface, where the administrators can easily control the class labels and classification context as well as export annotations.} 
% \label{fig:annotation} 
% \end{figure*}

\section{Resources and Dataset Contributions}
\noindent\textbf{Pretrained word embeddings for Sanskrit:}
There are two types of embedding methods: static and contextualized. Table \ref{tab:introTable} shows how they are categorized based on the smallest unit of input to the embedding model, such as character, subword, or token level. The paper focuses on two token-level word embeddings: \newcite[word2vec]{mikolov2013distributed} and \newcite[GloVe]{pennington-etal-2014-glove}. Word2vec is the foundation for all subsequent embeddings and works on the local context window, while GloVe considers the global context.
\begin{table}[!h]
\centering
\resizebox{0.45\textwidth}{!}{%
\begin{tabular}{|c|c|c|}
\hline
\textbf{Class}  & \textbf{Input type} & \textbf{Systems}    \\ \hline
Static   & character & charLM    \\ \hline 
   & subword & fastText    \\ \hline
   & token & word2vec, gloVe, LCM    \\ \hline\hline

Contextualized   & character & ELMo    \\ \hline
                & subword & ALBERT   \\ \hline 

\end{tabular}%
}
\caption{Overview of Sanskrit pretrained embeddings.}
\label{tab:introTable}
\end{table}
% However, these token-based embeddings have two limitations: (1) they can't represent words that aren't encountered during training (Out-of-vocabulary or OOV), and (2) they provide a single representation for all meanings of a word (Polysemy). 
To address the OOV issue, subword \cite{wieting-etal-2016-charagram,bojanowski-etal-2017-enriching,heinzerling-strube-2018-bpemb} and character-level \cite{kim_charLM,jozefowicz2016exploring}  modeling have been proposed. 
% Contextualized embeddings, on the other hand, help mitigate the polysemy problem by representing a word based on the complete sentence input.
We also explore two contextualized embeddings: ELMo \cite{elmo} and ALBERT \cite{ALBERT:}, a lighter version of BERT. 
We trained these 6 embedding methods on Sanskrit corpora and made the pretrained models publicly available \cite{sandhan-etal-2023-evaluating}.\footnote{\url{https://github.com/Jivnesh/SanskritShala/tree/master/EvalSan}}  The following section describes our proposed pretraining for low-resource settings.


\noindent\textbf{LCM Pretraining:}
 % \newcite[LCM]{sandhan-etal-2021-little} focused on a low-resource dependency parsing scenario, where obtaining morphological information is troublesome. To mitigate this challenge,
 We propose a supervised pretraining, which automatically leverages morphological information using the pretrained encoders.
In a nutshell, LCM integrates word representations from multiple encoders trained on three independent auxiliary tasks into the encoder of the neural dependency parser. LCM follows a pipeline-based approach consisting of two steps: pretraining and integration. Pretraining uses a sequence labelling paradigm and trains encoders for three independent auxiliary tasks. Later, these pretrained encoders are combined with the encoder of the neural parser via a gating mechanism similar to ~\newcite{sato-etal-2017-adversarial}. The LCM consists of three sequence labelling-based auxiliary tasks, namely, predicting the dependency label between a modifier-modified pair (\textbf{LT}), the monolithic morphological label \textbf{(MT)}, and the case attribute of each nominal \textbf{(CT)}.
% Each auxiliary task uses the same neural architecture and hyper-parameter settings. The only difference is in the output tags.
 % The neural architecture employed for these auxiliary tasks consists of BiLSTM encoders similar to \newcite{DBLP:conf/iclr/DozatM17} and a decoder with two fully connected layers followed by a softmax layer. 
 We encourage readers to refer \newcite[LCM]{sandhan-etal-2021-little} for more details.


The quality of word embedding spaces is evaluated through intrinsic and extrinsic methods. This study focuses on intrinsic evaluation, which involves assessing semantic and syntactic information in the words without testing on NLP applications. It is based on works such as \newcite{mikolov2013distributed} and \newcite{baroni-etal-2014-dont}.
These evaluations require a query inventory containing a query word and a related target word. However, such query inventories are not readily available for Sanskrit. To address this, we annotated query inventories for 4 intrinsic tasks: analogy prediction, synonym detection, relatedness, and concept categorization. The inventories were constructed using resources such as Sanskrit WordNet \cite{Kulkarni2017}, Amarako\d{s}a  \cite{inproceedings_nair}, and Sanskrit Heritage Reader \cite{goyaldesign16,heut_13}. 

 \noindent\textbf{Intrinsic evaluation testbed for Sanskrit word embeddings:}
The quality of word embedding spaces is evaluated through intrinsic and extrinsic methods. This study focuses on intrinsic evaluation, which involves assessing semantic and syntactic information in the words without testing on NLP applications. It is based on works such as \newcite{mikolov2013distributed} and \newcite{baroni-etal-2014-dont}.
% There are two primary methods for evaluating the quality of word embedding spaces in academic literature: intrinsic evaluation and extrinsic evaluation. This study focuses on intrinsic evaluation methods. 
% % Intrinsic evaluation involves assessing the quality of a word embedding space without testing it on downstream NLP applications. It evaluates the presence of semantic and syntactic information in the words, as described in works such as  \newcite{mikolov2013distributed} and \newcite{baroni-etal-2014-dont}.
These evaluations require a query inventory containing a query word and a related target word. However, such query inventories are not readily available for Sanskrit. To address this, we annotated query inventories for 4 intrinsic tasks: analogy prediction, synonym detection, relatedness, and concept categorization. The inventories were constructed using resources such as Sanskrit WordNet \cite{Kulkarni2017}, Amarako\d{s}a  \cite{inproceedings_nair}, and Sanskrit Heritage Reader \cite{goyaldesign16,heut_13}. 
% Intrinsic evaluation methods give insight into the effectiveness of different word embeddings, but it should not be taken as a sole measure of quality.


% \noindent\textbf{Compound dataset for Marathi:}
% \label{marathi_annotation}
% We have built a user-friendly annotation tool for general-purpose classification tasks. The tool is a Flask-based \cite{ronacher2011flask}  user-friendly web application styled by Bootstrap 5, and sports a simple administrative interface that lets the administrators easily control the class labels and classification context as well as export annotations.
% Figure~\ref{fig:annotation} shows our web-based mobile friendly annotation interface, where the task is to select the correct option from multiple-choices for the given compound with the context.  There are 4 broad categories of semantic types in Marathi. In case of confusion, we gave additional option to mark as {\sl ``Not sure''}. We also provide an option to add a comment to convey additional information about ambiguity or the concern for the corresponding example.


\noindent\textbf{Prabhupadavani Speech Translation Dataset:}
\label{intro}
% \begin{itemize}
%     \item Explain what is ST? Why this problem is interesting? Cascade vs End2end: gap is closed.
%     \item Code-mixing is ubiquitous. Why its important to address? How existing models are not adequate? How surge of datasets/models is coming from this direction.
%     \item But there are no such efforts in this direction for ST due to lack of data availability. How are we filling this gap? Our contribution: Speech Translation, ASR and MT data. What are the uniqueness of our data? 
% \end{itemize}
Speech Translation (ST) is a task in which speech is simultaneously translated from source language to a different target language.\footnote{We refer to speech translation as a speech-to-text task.} It aids to overcome the language barriers across different communities for various applications such as social media, education, tourism, medical etc. 

% models were although better than traditional methods due to above reasons but kept underperforming comparitive to cascaded approach. \cite{jan2019iwslt} and \cite{cettolo2016iwslt} were able to fill the gap to a certain extent between the performance of both these approaches.
%  was eventually able to perform similar to best cascaded model and hence the gap was filled leading to betterment in both architecture and performance. This embarked the increase in research in this field to improve the performance of these models. There was also a need of generating SLT specific dataset. Unavailability of training corpora has been one of the major obstacles in improvement of SLT models.

Nowadays, most users prefer to communicate using a mixture of two or many languages on platforms such as social media, online blogs, chatbots, etc. Thus, code-mixing has become ubiquitous in all kinds of Natural Language Processing (NLP) resources/tasks \cite{khanuja2020new,chakravarthi2020corpus,singh2018twitter,singh2018named,dhar2018enabling}.  However, the existing NLP tools may not be robust enough to address this phenomenon of code-mixing for various downstream NLP applications \cite{srivastava2021challenges}. Therefore, there has been a surge in creating code-mixed datasets: (1) to understand reasons for the failure of existing models, and (2) to empower existing models for overcoming this phenomenon. Nevertheless, it is challenging to find natural resources that essentially capture different aspects of code-mixing for creating datasets for a wide range of NLP tasks.
Although there has been considerable research in generating copious data and novel architectures for the ST task, we find that not much attention has been given to address the code-mixing phenomenon on the ST task. Possibly, this can be justified due to the lack of a code-mixed ST dataset.
%  for dealing with SLT but they lack one major thing which we wish to introduce in this paper, i.e., \textbf{code-mixing}.
To the best of our knowledge, no such sufficiently large, multi-lingual, code-mixed dataset is available for the ST. 
%  Generic monolingual and even multilingual systems have failed over code-mixed datasetes which has grabbed the attention of NLP and especially Speech Researchers. \\\\

Thus, in this work, we introduce \textbf{Prabhupadavani}, a multi-lingual, multi-domain, speech translation dataset for 25 languages containing 94 hours of speech by 130 speakers. The Prabhupadavani is about Vedic culture and heritage from Indic literature, where code-switching in the case of quotation from literature is important in the context of humanities teaching. The multiple domains cover utterances from public lectures, conversations, debates, and interviews on various social issues.
This is the first code-mixed data for speech translation to the best of our knowledge. It is code-mixed with English, Bengali and Sanskrit. From the typological point of view, the languages covered vary over ten language families. All the audios files have been manually aligned and translated. 
 We believe that our work will ignite research in this direction to understand- (1) How to make existing systems robust for handling this phenomenon effectively? (2) Can multi-lingual training help to improve performance on code-mixed speech translation? (3) Will the gap between the cascade and end-to-end systems be closed? 

% In the rest of the paper, Section 2 contains the related work that has been done in Speech Translation and Code-mixing. Subsequently, Section 3 gives description of the dataset including its thorough analysis in terms of both Speech Translation and Code-mixing. In this section, we've also shown linguistic analysis of all the languages present in our dataset which tells about how they are differentiated typologically. To be Continued once completed .....
% (1) What is the problem?
% (2) Why is it interesting and important?
% (3) Why is it hard? (E.g., why do naive approaches fail?)
% (4) Why hasn't it been solved before? (Or, what's wrong with previous proposed solutions? How does mine differ?)



% \begin{figure*}[!tbh]
% \centering
% \subfigure[\label{fig:tagging_schem}]{\includegraphics[width=0.5\linewidth]{images/DCST-AACL.pdf}}
% \subfigure[\label{fig:gating}]{\includegraphics[width=0.5\linewidth]{images/Gating-AACL.pdf}}
% \caption{Illustration of proposed architecture for a Sanskrit sequence. English translation: ``Demigods and demons had tried with equal effort for these planets". (a) Pretraining step: For an input word sequence, tagger predicts labels as per three proposed auxiliary tasks, namely, Morphological Tag (green), Case Tag (red) and Label Tag (black). (b) Parser with gating: $E^{(P)}$ is encoder of a neural parser like~\newcite{DBLP:conf/iclr/DozatM17} and $E^{(1)-(3)}$ are the encoders pre-trained with proposed auxiliary tasks. 
% % Gating mechanism outputs the combined representation of all the encoders. Finally, this enriched representation 
% Gating mechanism combines representations of all the encoders which,
% for each word pair, is passed to two MLPs to predict the probability of arc score (S) and label (L).
% }
% \label{fig:model}
% \end{figure*}
% \begin{table}[h]
% \centering
% \begin{small}
% \resizebox{0.9\textwidth}{!}{%
% \begin{tabular}{l|rcccc}
% \hline
% \textbf{Languages} & \multicolumn{1}{l}{\textbf{\# Types}} & \multicolumn{1}{l}{\textbf{\# Tokens}} & \multicolumn{1}{l}{\textbf{Types per line}} & \multicolumn{1}{l}{\textbf{Tokens per line}} & \multicolumn{1}{l}{\textbf{Avg. token length}} \\
% \hline
% English            & 40,324                               & 601,889                               & 10.58                                       & 11.27                                        & 4.92                                           \\
% French (France)    & 50,510                               & 645,651                               & 11.38                                       & 12.09                                        & 5.08                                           \\
% German             & 50,748                               & 584,575                               & 10.44                                       & 10.95                                        & 5.57                                           \\
% Gujarati           & 41,959                               & 584,989                               & 10.37                                       & 10.95                                        & 4.46                                           \\
% Hindi              & 29,744                               & 716,800                               & 12.36                                       & 13.42                                        & 3.74                                           \\
% Hungarian          & 84,872                               & 506,608                               & 9.13                                        & 9.49                                         & 5.89                                           \\
% Indonesian         & 39,365                               & 653,374                               & 11.54                                       & 12.23                                        & 6.14                                           \\
% Italian            & 52,372                               & 512,061                               & 9.23                                        & 9.59                                         & 5.37                                           \\
% Latvian            & 70,040                               & 477,106                               & 8.69                                        & 8.93                                         & 5.72                                           \\
% Lithuanian         & 75,222                               & 491,558                               & 8.92                                        & 9.20                                         & 6.04                                           \\
% Nepali             & 52,630                               & 570,268                               & 10.03                                       & 10.68                                        & 4.88                                           \\
% Persian (Farsi)    & 51,722                               & 598,096                               & 10.61                                       & 11.20                                        & 4.10                                           \\
% Polish             & 71,662                               & 494,263                               & 8.99                                        & 9.25                                         & 5.86                                           \\
% Portuguese(Brazil) & 50,087                               & 608,432                               & 10.80                                       & 11.39                                        & 5.12                                           \\
% Russian            & 72,162                               & 490,908                               & 8.96                                        & 9.19                                         & 5.79                                           \\
% Slovak             & 73,789                               & 520,465                               & 9.39                                        & 9.75                                         & 5.37                                           \\
% Slovenian          & 68,619                               & 516,649                               & 9.35                                        & 9.67                                         & 5.30                                           \\
% Spanish            & 49,806                               & 608,868                               & 10.75                                       & 11.40                                        & 5.07                                           \\
% Swedish            & 48,233                               & 581,751                               & 10.31                                       & 10.89                                        & 5.00                                           \\
% Tamil              & 84,183                               & 460,678                               & 8.37                                        & 8.63                                         & 7.65                                           \\
% Telugu             & 72,006                               & 464,665                               & 8.34                                        & 8.70                                         & 6.56                                           \\
% Turkish            & 78,957                               & 453,521                               & 8.27                                        & 8.49                                         & 6.35                                           \\
% Bulgarian          & 60,712                               & 564,150                               & 10.10                                       & 10.56                                        & 5.24                                           \\
% Croatian           & 73,075                               & 531,326                               & 9.58                                        & 9.95                                         & 5.28                                           \\
% Danish             & 50,170                               & 587,253                               & 10.40                                       & 11.00                                        & 4.98                                           \\
% Dutch              & 42,716                               & 595,464                               & 10.52                                       & 11.15                                        & 5.05      
%                             \\
% \hline
% \end{tabular}}
%  \end{small}
% \caption{Statistics of the \textbf{Prabhupadavani} dataset}
% \end{table}


% \subsection{Resource:} Vanimedia's Multi-language Subtitle Project\footnote{\url{https://vanimedia.org/wiki/Multi-language_Subtitle_Project}} has created 1,080 audio mini-clips of \'{S}r\={i}la Prabhup\={a}da's lectures, conversations, debates, interviews and is now transcribing them in multiple languages.\footnote{\url{https://vanimedia.org/wiki/Table:_Clips_to_subtitle}}
% % \'{S}r\={i}la Prabhup\={a}da is the founder of International Society of K\d{r}\d{s}\d{n}a Consciousness society.
% 700+ translators participate in creating subtitles for all 1,080 mini-clips for 108+ languages. Currently, this work has been completed for 25 languages. To procure subtitles for each clip in multiple languages, translators are provided with mini-clips and English subtitles that are manually aligned with each utterance. They use a third-party software named Dotsub.com\footnote{\url{https://dotsub.com}} and the task of translators is to provide translation for the corresponding utterance with the help of given transcription. 
% % Since the speaker here is speaking in conversational English, Google translate has been used in some cases to reduce the effort.
% % We would like to acknowledge the efforts of translators from different countries for translating all clips (1080) into over 495 languages. Most of the translation has been done manually. 
% On average, there are 3-4 translators for each language, and each clip takes more or less one hour for translation. Each translator has invested an average of 6 hours every day in translating these clips. Collectively, the time taken to translate 1,080 clips into 25 languages is over 45 weeks. 
% % To make the process of downloading subtitles automated and less time-consuming, we used selenium as a web crawler tool. 
% Current release of the dataset contains 25 languages (including transcription) for which transcription/translations are available. For these languages, we have over 53K utterances of transcription and translations. 
% % Table ~\ref{table:source-target-examples} illustrates an example from Prabhupadavani. 
% % The process of crawling and downloading all these translations took around a day while preprocessing them and making the data suitable for modeling took half a day more or less.
% \begin{table}[t]
% \begin{small}
% \centering
% \begin{tabular}{|c|c|c|c|}
% \hline
% \textbf{Language} & \textbf{Tokens} & \textbf{Types} & \textbf{Percentage} \\
% \hline
% English           & 500,136              & 6,312                 & 83.6                \\
% Bengali           & 46,933               & 3,907                 & 7.84                \\
% Sanskrit          & 51,246               & 7,202                 & 8.56                \\
% \hline
% \textbf{Total}    & 598,315              & 17,421                & 100                \\
% \hline
% \end{tabular}
% \caption{Statistics of code-mixing in \textbf{Prabhupadavani}}
% \label{table:statistics}
% \end{small}
% \end{table}

% \subsection{Preprocessing:}
% % Prabhupadavani has variety of distinguishable features like variety of speakers, their different accents, speeches in 3 languages, manually transcripted and translated speeches. The generation of such dataset required several steps.
% % \js{No information about the audio is given in the text. Please include some relevant information such as the sampling frequency, format and duration statistics.}
% In this section, we describe pre-processing steps followed to arrive at the final version of the data.
% First, we scrape transcription and their translations in 25 languages from Dotsub and extracted the corresponding Youtube links of all audio clips. We use Selenium\footnote{\url{https://www.selenium.dev/}} web crawler to automatize the process of downloading. We convert those videos into MP3 audio clips using a third-party application\footnote{\url{https://ytmp3.cc/uu100cc/}}. We chop the converted audio files based on the timestamps provided in the subtitle (.srt) files.\footnote{\url{https://pypi.org/project/audioclipextractor/}} This process boils down to 53,000 utterances with their transcription and translation in 25 languages. Table ~\ref{table:source-target-examples} illustrates the example from Prabhupadavani. In order to obliviate time and efforts needed for data pre-processing, we provide train, dev and test set splits using stratified sampling. There are 51,000, 1,000 and 1,000 utterances in train, dev and test set, respectively. We consider the following dimensions for stratified sampling: (1) different speakers (2) proportion of intra-sentential and inter-sentential code-mixing.
% \begin{table}[t]
% \begin{tiny}
% \centering
% \begin{tabular}{|c|c|c|}
% \hline
% \textbf{Language} &\textbf{Type} & \textbf{Examples}\\
% \hline
% English-Sanskrit& Inter & K\d{r}\d{s}\d{n}a is assuring. \textcolor{red}{aha\.{m} tv\={a}\.{m} sarva-p\={a}pebhyo mok\d{s}ayi\d{s}y\={a}mi} \\
% &Intra&Sense gratification means \textcolor{red}{udara-upastha-jihv\={a}}\\
% \hline
% % Hindi & इसलिए, अंत में कृष्ण कहते हैं, सर्व धर्मान परित्यज्य\\
% Sanskrit-English&Inter&\textcolor{red}{\={I}\`{s}\={a}v\={a}syam ida\.{m} sarvam}. Everything belongs to God \\
% &Intra&\textcolor{red}{andh\={a} yath\={a}ndhair upan\={i}yam\={a}n\={a}\d{h}} and people, leaders. \\ \hline
% English-Bengali&Inter&Give up their. \textcolor{violet}{Asat-sa\.{n}ga-ty\={a}ga ei vai\d{s}\d{n}ava \={a}c\={a}ra}\\
% &Intra& Therefore Caitanya Mah\={a}prabhu said \textcolor{violet}{guru-k\d{r}\d{s}\d{n}a-k\d{r}p\={a}ya}\\ \hline
% Bengali-English&Inter&\textcolor{violet}{Guru-k\d{r}\d{s}\d{n}a-k\d{r}p\={a}ya p\={a}ya bhakti-lat\={a}-b\={i}ja}. Then our devotional service is perfect\\
% &Intra&\textcolor{violet}{t\={a}\.{n}h\={a}ra n\={a}hika do\d{s}a} means he is not faulty.\\\hline
% \end{tabular}
% \caption{Examples of code-mixing in \textbf{Prabhupadavani}. English, Sanskrit and Bengali are indicated by black, red and violet color, respectively.}
% \label{table:code-mixed_examples}
% \end{tiny}
% \end{table}
% \begin{table}[t]
% \begin{small}
% \centering
% \begin{tabular}{|c|c|c|}
% \hline
% \textbf{} &\textbf{Language} & \textbf{Translations}\\
% \hline
% Source& English &You can become Brahman. Brahma-bh\={u}y\={a}ya kalpate  \\ \hline
% % Target&Hindi&तुम ब्रह्म बन सकते हो । ब्रह्मभूयाय कल्पते ।\\
% Target& Bulgarian &\includegraphics[width=0.45\textwidth]{images/balgarian.png}\\
% & Hindi &\includegraphics[width=0.4\textwidth, height=0.35cm]{images/hindi.png}\\
% & Russian &\includegraphics[width=0.45\textwidth]{images/russian.png}\\
% & Tamil &\includegraphics[width=0.45\textwidth]{images/Tamil.png}\\
% & Gujarati &\includegraphics[width=0.45\textwidth, height=0.35cm]{images/gujarati.png}\\
% % &Bulgarian&Можете да станете Брахман. Брахма бхуяя калпате.\\
% % &Russian&Вы можете стать "Брахманом". "Брахма-бхуйайа калпате"\\
% % &Tamil&நீ ப்ரம்மன் ஆகலாம். ப்ரம்ம-பூயாய-கல்பதே'.\\
% % &Gujarati&તમે બ્રહ્મ બની શકો છો.બ્રહ્મ-ભૂયાય-કલ્પતે.\\
% \hline
% \end{tabular}
% \caption{Sample data point from \textbf{Prabhupadavani}. For a code-mixed utterance, we show its English transcription (source) and the corresponding translations for 5 languages.}
% \label{table:source-target-examples}
% \end{small}
% \end{table}

% \subsection{Code-mixing:} 
% Prabhupadavani is code-mixed across three languages: English, Sanskrit, and Bengali. Table~\ref{table:statistics} reports the overall statistics of the code-mixing present in Prabhupadavani. If we consider the number of tokens in utterances, then it is mainly dominated by English (83.0\%) tokens; however, it is not the case in terms of a number of types. This attributes to the contrasting nature of morphology (English vs Sanskrit/Bengali).
% % Code-mixing in Prabhupadavani is precisely in 3 languages namely English, Bengali and Sanskrit among which English is the dominant one (see Table \ref{table:statistics}). 
% Code-mixing is categorized into two classes- (1) inter-sentential: speaker chooses to switch the language after completion of utterance (2) intra-sentential: speaker switches the language within an utterance. Table \ref{table:code-mixed_examples} illustrates examples of code-mixing from Prabhupadavani. Table \ref{table:ablation_train_size} shows the statistics of both these types of code-mixing.
% Mainly speaker explains Sanskrit verses to the English audience; therefore, transitions between the Sanskrit-English pair is more. However, sometimes speaker also use Bengali literature to illustrate the points. Thus, we observe Bengali-English code-switching. Notably, there is no code-switching between Bengali-Sanskrit because the audience is English speaking.


% % English-Sanskrit and vice versa are the dominant one here because the speakers are native to both these languages. All the śloka\footnote{Shloka or śloka is a poetic form used in Sanskrit, the classical language of India.} in the speech are precisely in Sanskrit and hence this large code-switching to Sanskrit. Bengali has been relatively less frequently used, mostly by third-party people. Nevertheless, amount of Bengali code-switching is more or less similar to Sanskrit due to diversity in our data which implies we've considered all the speakers in our speech data equally and hence there is diversity of speakers, the language they're speaking and language they are switching into.
%  \begin{table}[h]
%   \begin{small}
% \centering
% \begin{tabular}{|c|c|c|}
% \hline
%      &\textbf{Inter-Sentential} & \textbf{Intra-Sentential}           \\
% \hline
% English-Sanskrit  & 2,356 & 2,338  \\
% Sanskrit-English  & 2366 & 851 \\
% English-Bengali  & 339 & 124 \\
% Bengali-English  & 339 & 0 \\
% \hline
% \end{tabular}
%     % \caption{Impact on performance as training sample size increases}
%     \caption{Code-Mixing type for our dataset}
%      \label{table:ablation_train_size}
%      \end{small}
% \end{table}

% \subsection{Language diversity:} From typological point of view, Prabhupadavani covers 25 languages (inlcluding ASR) from 10 language families. They are listed as follows:
% (1) \textit{Indo-European:-}
% (a) \textit{Romance:}  Italian, Portuguese, Spanish, French
% (b) \textit{Germanic:}  German, Swedish, Danish, Dutch, English
% (c) \textit{Baltic:} Lithuanian, Latvian 
% (d) \textit{Slavic:} Croatian, Polish, Slovak, Russian, Slovenian, Bulgarian, 
% (e) \textit{Indo-Aryan:} Bengali, Hindi, Sanskrit, Nepali
% (f) \textit{Indo-Iranian:} Persian (Farsi)
% (2) \textit{Uralic:-}
% (a) \textit{Finno-Ugric:} Hungarian
% (3) \textit{Austronesian:-}
% (a) \textit{Malayo-Polynesian:} Indonesian
% (4) \textit{Dravidian:-}
% Tamil, Telugu.
% % The languages that are extracted for training are diverse from their typological point of view.
% Prabhupadavani contains fusional languages: Indo-European, Uralic and Agglutinative languages: Austronesian (Indonesian), Dravidian and Turkic (Turkish). In the former languages, grammatical markers bear several meanings and for the latter ones, they exhibit only one meaning at the same time.
% Except Hindi (Indo-Aryan), all the languages in our dataset use nominative-accusative marking. Hindi uses ergative-absolutive marking upto a limited extent. 
% % In the ergative-absolutive marking, the subject of an intransitive verb and the patient of a transitive verb are handled similarly and get the same case marker. 
% % However, the agent of a transitive verb is treated differently than the subject of an intransitive verb.
% % In case of Hindi, ergative alignment occurs only when the verb is in the perfective aspect for transitive verbs.
% We can also categorize languages based on the number of grammatical genders. Some languages pose (1) three genders: German, Russian, Swedish, etc. (2) two genders: French, Spain, Hindi, etc. (3) no genders: English, Nepali, Persian, Turkish, etc.
% % Another interesting linguistic phenomena in which the dataset is diversified is the grammatical genders. Some languages only contain two genders (Masculine \& Feminine), some contain three (including Neutral), and others do not possess grammatical genders.
% % Indo-European languages like  are two-gender languages. are three-gender while  have no gender distinction at all. are further examples of having more than three grammatical genders. 
% Based on a syntactic construct, we can categorize the languages present in Prabhupadavani- (1) SVO word order: English, Italian, French, Indonesian, etc. (2) SOV word order: Indo-Aryan, Dravidian and Turkic (3) flexible word order: Russian, Hungarian.

% Thus, the diversified language coverage of \textbf{Prabhupadavani} along with its code-mixed nature makes it a suitable dataset to investigate various linguistic phenomena for the speech translation task, ASR and machine translation. 
% % \js{Give example from the dataset and have a separate section where u talk about application of dataset.}
% % We believe that this dataset can be widely used for speech-related tasks like Speech Recognition (both Cascade and end-to-end models), Automatic linguistic feature detection, language identification in speeches etc. 
% % In the consequent Section 4, we've shown the baseline models being used, their experimental results on the trained end-to-end SLT model and thorough error analysis of the model. 

% \subsection{Applications of dataset:}
% In this section, we throw some light on possible applications of Prabhupadavani: (1) The full dataset of Prabhupadavani contains 2,400 hours of speech. The current release of Prabhupadavani dataset can be utilized to facilitate automatic subtitling of the remaining part of data in the different languages. In this way, it will also be helpful to generate relatively larger dataset.
% % (2) Our dataset has corresponding translations paralleled available for all 25 languages. Therefore, with the help of our dataset, a single model can be built to translate speech into multiple languages.
% (2) This dataset can provide a fertile soil to investigate on- How to make existing systems robust to code-mixing phenomenon? Will the gap between cascade and end-to-end to approaches be closed? Can multi-lingual training help to address code-mixing phenomenon? Can we train single ST system for all languages? How robust will be these models on another domain? 

 
% We investigate the efficacy of embeddings approaches (originally proposed for languages other than Sanskrit) for Sanskrit along with various challenges posed by language.
% \footnote{Our code, data and trained models are  publicly available at: \url{https://github.com/jivnesh/EvalSan}}


% \section{Intrinsic evaluation datasets}
% \label{intro}
% The supervised learning paradigm has shown remarkable performance in many downstream Natural Language Processing (NLP) tasks. In this domain, the NLP community has witnessed the emergence of neural-based approaches with the state of the art performance.  The dramatic popularity of such approaches has garnered considerable attention from Sanskrit Computational Linguistics (SCL) community. The primary prerequisite for the feasibility of such approaches is the availability of task-specific labeled data. Therefore, as a first step, there was a need for preparing such task-specific resources. As a result, laudable efforts have been put by the community for building task-specific labeled data for various NLP tasks \cite{krishna-etal-2017-dataset,hellwig-nehrdich-2018-sanskrit,hellwig-etal-2020-treebank}. The availability of such resources triggered the emergence of the data-driven neural-based approaches into the SCL field. The wide success of neural-based data-driven approaches is greatly justified by the state of the art performance for many downstream tasks for Sanskrit, namely, segmentation \cite{hellwig-nehrdich-2018-sanskrit,reddy-etal-2018-building,krishna-etal-2018-free}, dependency parsing \cite{amrith21,krishna2020neural,sandhan2021little,krishna-etal-2020-keep}, semantic type identification \cite{sandhan-etal-2019-revisiting,krishna-etal-2016-compound}, word order linearisation \cite{krishna-etal-2019-poetry,amrith21} and morphological parsing \cite{gupta-etal-2020-evaluating,krishna-etal-2018-free}. 

% The supervised approaches have shown remarkable performance in several downstream NLP tasks and many of these use word embeddings as a primary component.
% % Especially, there are many NLP domains where such labelled data is not available for Sanskrit language. The transfer learning approaches are new kids in the NLP field to mitigate the massive task-specific data bottleneck. The transfer learning is set of methods that leverage readily available unlabelled data in various domains and tasks to improve the task-specific performance \cite{ruder-etal-2019-transfer}. 
% In 2013, \newcite{mikolov2013distributed} proposed a new milestone in the field of word embedding, which completely revolutionized Natural Language Processing (NLP). From there, word embedding has been a buzzword in NLP and has become part and parcel of downstream applications.  These word embedding approaches adopt a semi-supervised learning paradigm. They do not depend on any explicitly labeled data or human supervision.  Availability of massive unlabelled corpora and ease of integration into downstream NLP tasks made them exciting for the researchers. Sanskrit, the cultural heritage of India, has 30 million extant manuscripts \cite{goyal-etal-2012-distributed}. Last decade, there has been much excitement in digitization for Sanskrit, as a result, we have DCS\footnote{\url{http://www.sanskrit-linguistics.org/dcs/index.php}}, The Sanskrit Library\footnote{\url{https://sanskritlibrary.org/}} and GRETIL\footnote{\url{http://gretil.sub.uni-goettingen.de/gretil.html}}. To reduce the labeled data dependency, it's crucial to take advantage of such cheaply available resources. 

% This motivates us to systematically investigate word embedding approaches that are originally proposed for resource-rich languages like English. Most of the research in NLP disproportionately focuses on resource-rich languages due to readily available language resources: digitized texts and gold standard labeled data \cite{joshi-etal-2020-state}. Also, the recent word embedding approaches have been studied for resource-rich languages such as English. However, such analysis is lacking for Sanskrit. 
% In addition to the morphological rich nature of language, the Sanskrit is a relatively free word order language, and most words are compound words (sam\={a}sa) that demand special attention for modeling the word embedding approach. To conduct a systematic study on the efficacy of these approaches, we categorize word embeddings into two categories, namely, \textit{static} and \textit{contextualized}. The \textit{static} embeddings generate a single representation for all the senses possible for a word, irrespective of surrounding context words. In contrast to that \textit{contextualized} embeddings generate a different representation for each sense of the meaning depending on the surrounding context words. This work provides fertile soil for investigating the following questions: (1) Which linguistic phenomenons are captured by word embeddings? (2) Out of existing word embedding approaches, which embeddings are most suitable for Sanskrit? (3) What are the shortcomings of existing approaches specific to Sanskrit?
% Based on our experiments, our major findings are as follows:
% \vspace{-1mm}
% \begin{enumerate}\itemsep0em
%     % \item The subword level segmentation with the \texttt{sentencepiece} model empowered the \texttt{word2vec} and \texttt{GloVe} to such an extent that it becomes almost competitive with \texttt{FastText} (Section \ref{experiments}).
%     \item Our intrinsic evaluation results illustrate that word embedding models trained on Sanskrit corpus are able to capture exceptionally good amount of the syntactic information. However, they perform relatively poorly with the semantic notion of relatedness - similarity mainly due to Out of vocabulary problem.
%     % \item The \textit{contextualized} embeddings get benefited by the explicit modelling of context during training for improving the performance of simple context independent tasks without providing context during evaluation (Section \ref{experiments}). 
%     \item The \textit{contextualized} word embedding model by \newcite{elmo} outperforms all the word embeddings in all the intrinsic tasks with a large margin except semantic categorization task (Section \ref{experiments}). We employ contextual models without a context to measure efficacy of these approaches compared to static approaches. Applying \textit{contextualized} models without context is similar to just using their underlying static word representation.
 
%     \item The qualitative analysis shows that the \textit{contextualized} representations generated by \newcite{elmo} and \newcite{ALBERT:} for polysemous words indicating the same sense of meaning forms a cluster for each sense of meaning (Section \ref{context_cluster}). This is indeed a serendipitous outcome for such data-hungry models when trained on negligibly small amount of corpus available for Sanskrit.
    
%     \item We release our codebase, datasets and models publicly at: \url{https://github.com/jivnesh/EvalSan}. This might help the research community to do further analysis and apply these embeddings to downstream NLP applications of Sanskrit.
%     % \item These tasks rely on query inventory datasets consisting query word and semantically related target word. These query inventories are readily available for resource rich languages but not for Sanskrit. We create such inventories for four different intrinsic tasks, namely, relatedness, synonym detection, analogy prediction and concept categorization,. For creating such query inventory dataset for these intrinsic evaluation tasks, we use \textit{Amarako\d{s}a}\footnote{\url{https://sanskrit.uohyd.ac.in/scl/amarakosha/index.html}} \cite{inproceedings_nair}, Sanskrit WordNet\footnote{\url{https://www.cfilt.iitb.ac.in/wordnet/webswn/index.php}} \cite{Kulkarni2017} and Sanskrit Heritage Reader\footnote{\url{https://sanskrit.inria.fr/DICO/reader.fr.html}} \cite{goyaldesign16,heut_13}
% \end{enumerate}

% %
% % The following footnote without marker is needed for the camera-ready
% % version of the paper.
% % 
% %\blfootnote{
%     %
%     % for review submission
%     %
% %}

% \subsection{Neural Word Embedding}
% Neural word embedding methods construct vector space so that semantically related words are projected in closer vicinity compared to unrelated words. Word embedding is a dense representation of words in low-dimensional vector space. It mainly exploits the distributional hypothesis: neighboring words share similar meaning \cite{firth1957synopsis,harris1954distributional}. 

% \begin{table}[!h]
% \centering
% \resizebox{0.6\textwidth}{!}{%
% \begin{tabular}{|l|l|l|}
% \hline
% % Parser & \begin{tabular}[c]{@{}l@{}}Parsing\\ Approach\end{tabular}&\begin{tabular}[c]{@{}l@{}}Learning\\ Framework\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Input \\ Representation\end{tabular}} \\ \hline
% \textbf{Category}  & \textbf{Input level} & \textbf{Models}    \\ \hline
% Static   & Token & Word2vec, GloVe    \\ \hline
%    & Subword & FastText    \\ \hline
%    & Character & CharLM    \\ \hline \hline

% Contextualized  & Subword & ALBERT   \\ \hline 
%  & Character & ELMo    \\ \hline
% \end{tabular}%
% }
% \caption{Categorization of embedding models}
% \label{tab:introTable}
% \end{table}

% As shown in Table \ref{tab:introTable}, we consider the two broader categories of embedding approaches, namely, \textit{static} and \textit{contextualized}. Further, we divide them based on an atomic unit of input fed to the model, i.e., token level, subword level and character level. First, we consider token level embeddings: \texttt{word2vec} \cite{mikolov2013distributed} and \texttt{GloVe} \cite{pennington-etal-2014-glove}. We consider \texttt{word2vec} as a strong baseline because it is the basic backbone of all the neural-based follow-up works in this domain. While \texttt{word2vec} focuses on the local context of a target word, \texttt{GloVe} is an alternative approach that considers the global context of a target word. Therefore, \texttt{GloVe} can be seen as representative of count-based models; hence we choose to include it in our study.  However, these token-based approaches suffer from two serious issues: (1) Out of vocabulary (OOV) problem: they fail to obtain representation for words which are not seen during training (2) Polysemy problem: a single representation for multiple meanings of words. In order to handle the first drawback, sub-word \cite{wieting-etal-2016-charagram,bojanowski-etal-2017-enriching,heinzerling-strube-2018-bpemb} and character level \cite{kim_charLM,jozefowicz2016exploring} compositional modeling is proposed. These models learn composition functions to obtain word-level representation of a word using character level or subword level modeling. In the next category, the advent of contextualized embeddings is attributed to the polysemy problem.
% % Although, sense embedding \cite{} is another alternative, but due to various challenges, it could not garnered much attention of researcher.
% % Earlier, \newcite{} embeddings were present in contextualized domain. 
% The year 2018 is an inflection point in the field of NLP with the launching of contextualized embedding by \newcite[\texttt{ELMo}]{elmo}. The specific meaning of the word can be understood by the context words surrounded by it. Hence, in contextualized embedding approach, the representation of each token word is a function of entire sentence as a input.
% % Unlike sense embedding, these models simply rely on readily available unlabelled data. We consider another representative of this category: Flair \cite{}.
% %  \texttt{ELMo} learns character level composition function to generate word representation.
%  The emergence of another contextual embedding by  \newcite[\texttt{BERT}]{bert} can be seen as a clever recipe of a bunch of excellent ideas bubbled in the field of NLP in recent years. 
% %  \texttt{BERT} \cite{bert} considers subword level composition function for a word.
%  We consider a derivative of \texttt{BERT} known as \texttt{ALBERT} \cite{ALBERT:} which is light version of \texttt{BERT} with relatively less number of parameters. 
% %  This momentous development enabled researchers to use this powerhouse as an off-the-shelf feature extractor: saving the training model's computational efforts from scratch.


% % Although, unsupervised learning, self-training, weakly supervised paradigms could reduce the dependence on labelled, one must have sufficient labelled data to evaluate the efficacy of trained system and massive unlabelled data to feed data hungry systems. 



% \noindent\textbf{Tokenizer:}
% Token-based word embeddings such as \texttt{word2vec} and \texttt{GloVe} suffer from OOV problem, i.e., they are not capable of producing vector representation for words that are not seen during training. Here, word is defined as a continuous unsandhied string separated by delimiter. This problem is even more prominent for Sanskrit due to the following reasons: (1) morphological-rich nature (2) highly inflectional (3) most of the text is available in \textit{sandhied} format. Hence, token-based approaches are highly ineffective for Sanskrit. We take inspiration from \newcite{heinzerling-strube-2018-bpemb} and leverage \texttt{sentencepiece} tokenizer \cite{sentencepiece} to overcome OOV problem. The \texttt{sentencepiece} is unsupervised tokenizer used for neural-based tasks such as machine translation and sequence generation task. This is a purely data-driven tokenizer and does not require any pretokenization. Also, this is language independent approach where words are considered as a sequence of unicode characters. The \texttt{sentencepiece} overcomes the challenge as mentioned earlier by creating a new vocabulary instead of relying on real word boundaries. This method uses a greedy approach to figure out subword units that maximize the likelihood of the language model \cite{sentencepiece}. There exist other unsupervised tokenizers such as \texttt{Wordpiece} \cite{wordpiece} and \texttt{BPE} \cite{bpe}. However, these approaches expect tokenized words as input and most of the available text for Sanskrit is in \textit{sandhied} format. Hence, \texttt{sentencepiece} is the most befitting choice as a tokenizer. We demonstrate \texttt{sentencepiece} tokenization with an example as shown below.\footnote{Originally, we apply tokenization on SLP1 transliterated data. Just to illustrate, we show an example in the romanized (IAST) transliteration scheme.} Here, \texttt{sentencepiece} considers space character as a normal character and is replaced by \say{\_} character. Note that \textit{ man\={a}\_bhava} is a word in our newly generated vocabulary, originally part of two words.
% \begin{center}
%    \textbf{Sandhied sentence (original)} \\
%    \textit{man-man\={a} bhava mad-bhakto mad-y\={a}jī m\={a}\.{m} namaskuru \\
% m\={a}m evai\d{s}yasi yuktvaivam \={a}tm\={a}na\.{m} mat-par\={a}ya\d{n}a\d{h}} \\
% \end{center}
% \begin{center}
%    \textbf{Segmented by \texttt{sentencepiece} tokenizer }\\
%    \textit{\_man - man\={a}\_bhava \hspace{0.1mm} \_mad -bhakto \hspace{0.1mm} \_mad - y\={a}jī \hspace{0.1mm} \_m\={a}\.{m} \hspace{0.1mm} \_namas kuru \\
% \_m\={a}m \hspace{0.1mm} \_evai \d{s}yasi \hspace{0.1mm} \_yukt vaivam \hspace{0.1mm} \_\={a}tm\={a}n a\.{m} \hspace{0.1mm} \_mat - par\={a}ya\d{n} a\d{h}} 
% \end{center}

% \subsection{Static Embeddings}
% \noindent\textbf{Word2Vec:}
% The work of \newcite{mikolov2013distributed} is a new milestone in the field of word embeddings and popularly known as \texttt{word2vec}. This work was the basic backbone of the neural-based word embedding approach, which led to many of word embedding variants tackling various challenges. This model exploits the distributional semantics hypothesis: \say{semantically similar words are used in similar contexts} \cite{firth1957synopsis,harris1954distributional}. \texttt{Word2vec} often considered as one of the seminal the deep learning models; however, technically, neither the architecture is deep, nor the model uses non-linearities. It adapts language modeling objectives to consider the additional context. Language modeling is the task where the next word is predicted given previous \textit{n} words. However, \texttt{word2vec} also considers next \textit{n} words as a context.  The basic intuition behind this model is to project the words into \textit{n} dimensional vector space such that semantically similar words are placed in closer vicinity than non-similar words. In other words, the dot product of similar (cosine similarity) words will be higher compare to that with non-similar words. In order to obtain geometric organization of words, authors propose two training methods: (1) Continuous Bag of Words \texttt{(CBOW)} (2) \texttt{Skip-gram}. While the \texttt{CBOW} uses context words to predict the target word, skip-gram predicts context words given the target word as an input. Note that context is considered as a window of \textit{n} words surrounding target word from forward and backward direction. Unlike prior sparse representations, these learned vector representations are dense vectors of dimension ranging from 50-1000 and these dimensions do not have clear semantic interpretation.

% \noindent\textbf{GloVe:} Prior to \newcite{mikolov2013distributed}, count-based models were prominent in the word embedding field. These count-based models  \cite{bengio2003neural,count_1,count_2} are explicitly designed to model the global statistics of a entire corpus. Predictive models such as \texttt{word2vec} solely focus on the target word's local context. To gain the best of two worlds, \newcite{pennington-etal-2014-glove} proposed an alternative word embedding technique that integrates global statistics via matrix factorization and local context via the sliding window method. This approach focuses on the co-occurrence of each word with all other words in the entire corpus, therefore called Global Vectors \texttt{(GloVe)}. For the unsupervised models, the primary source of information to learn word representation is corpus statistics. However, how to exploit corpus statistics to generate word representations is an interesting problem. \newcite{pennington-etal-2014-glove} show that the ratio of co-occurrence probabilities of words is more indicative of their relation than a direct co-occurrence probability . 
% % Here, $P(A,B)$ is given by $X_{AB}/X_{A}$ where $X_{AB}$ is the number of times word $A$ co-occurs with word $B$ and $X_{A}$ is the total number of times word $A$ appears in the corpus. How can we use scalar quantity $P(A,C)/P(B,C)$ to learn meaningful vector representation of words?  \newcite{pennington-etal-2014-glove} propose a novel objective function to tackle this challenge.\footnote{We recommend the readers to refer original paper for derivation details of objective function.} The training objective of this model is to learn word vectors for words A and C such that their dot product gives a fair estimate of their co-occurrence counts. Formally, the objective can be expressed as follows: 
% % \[A^TC+b_{A}+b_{C}=log(X_{AC})\]
% % In the above equation, $b_{A}$ and $b_{C}$ are bias terms for the words A and C, respectively.  The generated vectors are considered as the final word embedding vectors for words A and C.
% Although, \texttt{GloVe} does not use neural network, \newcite{levy-etal-2015-improving} consider it as a predictive model due to following reason:  Unlike other count-based models, \texttt{GloVe} use the Stochastic Gradient Descent (SGD) optimization for non-convex objective function. The \texttt{GloVe} outperforms it's peer models (including \texttt{word2vec}) in several intrinsic and extrinsic evaluation tasks. The model works well with a small-sized corpus but is highly scalable to a larger corpus. Although the model demands much memory to populate the co-occurrence matrix in large corpora, the authors term it as a \say{one-time, up-front cost}.

% \noindent\textbf{FastText:}
% Token-level embeddings like \texttt{word2vec} and \texttt{GloVe} suffer from \textit{Out of Vocabulary} (OOV) problem. That means these models cannot generate vector representation for words that are not present in vocabulary. For example, even if model learns embeddings for \textit{p\={a}cik\={a}} and \textit{bh\={a}rya\d{h}}, it will not be able to handle the word \textit{p\={a}cik\={a}bh\={a}rya\d{h}}, if it is not a part of vocabulary. Hence, such approaches could not serve the need of morphologically rich languages. Also, the model is not capable of handling different possible inflections of a word (for example, \textit{r\={a}ma\d{h}, r\={a}m\={a}bhy\={a}m, r\={a}masya}) if such inflectional variants are not a part of the vocabulary. Hence, to overcome these shortcomings, \newcite[\texttt{FastText}]{bojanowski-etal-2017-enriching} proposed a new word embedding technique, specifically, for learning reliable representations for OOV words. To accomplish this, the authors propose to incorporate subword level information into the model. While learning vector representation of target word, simultaneously, representations of all n-grams (\textit{n} varies from 3 to 6) are also learned. For example, for n=4, the possible 4-grams of a word \textit{ajñ\={a}nam} are \textit{<ajñ, jñ\={a}na, ñ\={a}nam, \={a}nam>}. The brackets are used for padding purposes to indicate the beginning and end of the word. With this modification, the training procedure similar to word2vec is applied. This subword level representation learning empowers the model to generate a representation for OOV words by simply summing representations of n-grams corresponding to the target word.  \texttt{FastText} has been shown to improve performance on syntactic word analogy tasks, especially in the case of morphologically rich languages.

% \noindent\textbf{CharLM:}
% \newcite[\texttt{CharLM}]{kim_charLM} proposed a new variant of language model that learns subword information through a character-level convolutional neural network (CNN). 
% % Language modeling is a task where the model predicts the next word given the \textit{n} previous context words. 
% In a standard neural language modeling setting, the model takes word-level vector representation as input and predicts word-level information. This modeling decision makes the model blind to subword information. For example, the inflected forms of a root word should have structurally similar word embeddings because they shared common sub-strings except for affixes.  Therefore, to capture subword level information, \texttt{CharLM} takes a character-level input and learns composition function to generate word-level representation. This is achieved by extracting the features from CNN followed by a highway network. Finally, these extracted features are fed to a long short-term memory (LSTM) recurrent neural network language model to make word-level predictions. \newcite{kim_charLM} argues that without using word embeddings as input to the language model, their model gets the additional advantage of fewer parameters with competitive performance. Also, they show that the model is capable of encoding both semantic and orthographic information. 
% % They demonstrate that languages with rich morphology outperform word-level/morpheme-level LSTM baseline methods. 


% \subsection{Contextualized Embedding}
%  Each word has multiple meanings and their uses highly depend on the context they are used. However, irrespective of context, traditional approaches give a single vector representation for a word. Therefore, traditional word embeddings are called \textit{static} embeddings. For example, there are two possible meanings of a word \textit{cakrī}: (1) a potter (2) the holder of the disc and its uses highly depends on the context. In order to solve this polysemy problem, contextualized embeddings like \texttt{ELMo} \cite{elmo} and \texttt{BERT} \cite{bert} are proposed. In literature, there exists two domains for applying language representations to downstream tasks, namely, \textit{feature-based} and \textit{fine-tuned}. The feature-based approach simply augments the learned representation into the task-specific model architecture and well-known example in this category \texttt{ELMo}. A fine-tuned approach such as \texttt{BERT}, integrates pretrained model architecture into task-specific model and trains all the parameters, including the pretrained component. The emergence of these embeddings is described as a beginning of a new era in a word embedding. Their exceptional popularity in the field launched many of contextualized embedding variants. Hence, we include \texttt{ELMo} and \texttt{ALBERT} (A Light \texttt{BERT}: derivative of \texttt{BERT} model with significantly less number of parameters) \cite{ALBERT:} in our study. From an architectural point of view, \texttt{ELMo} belongs to LSTM based language model family and \texttt{ALBERT} belongs to the transformer-based language model family. 

% \noindent\textbf{ELMo:}
% % The most compelling signs of \texttt{ELMo} in NLP are mainly attributed to ease of integration and stunning improvement in the state of the art performance for many Natural Language Understanding tasks.
% Unlike traditional \textit{static} word embeddings, \texttt{ELMo} computes a representation of each token word as a function of all the words in a sentence. Authors employ the language modeling objective; hence, these representations are also called as \texttt{ELMo} (Embeddings from Language Models). There are three salient features of \texttt{ELMo}: (1) \textit{contextual:} the word representation depends on surrounding context words (2) \textit{deep:} the word representation is weighted average of all the layers of model architecture  (3) \textit{character based:} character based modeling enables model to encode morphological clues to obtain robust representations for OOV words, especially, for languages with rich morphology.
% Prior state of the art neural language models \cite{kim_charLM,jozefowicz2016exploring} takes context-independent token-level representation as an input to forward language modeling objective where next word is predicted based on previous \textit{n} words. Similarly, the backward language model predicts a word given \textit{n} following words, i.e., precisely opposite to the forward model. \texttt{ELMo} coupled both forward and backward language model objective function together.
%  Through ablations and intrinsic evaluation experiments, authors discover that higher-level layers in model architecture capture semantic properties and lower-level layers are syntactic. They show that a linear combination of internal representation helps obtain a rich representation, which is a better decision over just using top layer representation. Simultaneously providing enriched representation via a weighted linear combination of all layers, the model can choose the most relevant features for specific downstream tasks.

% \noindent\textbf{ALBERT:}
%  \texttt{BERT} is blend of several clever ideas that has been emerging in the field of NLP such as semi-supervised learning \cite{dai2015semisupervised}, \texttt{ELMO} \cite{elmo}, \texttt{ULMFIT} \cite{ulmfit} and \texttt{Transformer} \cite{attention_vaswani}.
% The foundational concept used in \texttt{BERT} is a transformer architecture popularized by \newcite{attention_vaswani}. Inspired from \newcite[\texttt{ULMFIT}]{ulmfit}, \texttt{BERT} adopts the fine-tuning approach to augment learned contextual representation in downstream applications. Authors argue that the previous language representations are unidirectional language modeling objective and this choice limits the model to learn effective representations. First, \texttt{ELMo} from the LSTM family demonstrated the effectiveness of a bidirectional language modeling for learning enriched representations. Suppose we introduce bidirectional language modeling into a transformer with a vanilla language modeling objective. In that case, the problem will become trivial and it will not be possible to learn robust representations. Therefore, to tackle this challenge, authors adapt a vanilla language modeling objective to a masked language objective. Here, instead of predicting the next word from previous \textit{n} words, the model masks a few words from a sentence and learns to recover masked words from the remaining words. This is also called a denoising objective. In this way, \texttt{BERT} can take advantage of the surrounding context from both sides simultaneously. 

% This data hungry model reports the state of the art results in many downstream tasks on the leaderboard at the expense of huge parameters. Despite the great success of \texttt{BERT}, it is highly impractical to train such a monstrous model with limited available resources for Sanskrit. For example, \texttt{BERT-base} has 110 million trainable parameters, making it computationally very intensive and nearly impossible to train on consumer devices. Therefore, we choose a derivative of \texttt{BERT} called as \texttt{ALBERT}, a light \texttt{BERT}, which has significantly few parameters than traditional \texttt{BERT} model with significantly better performance. The authors achieved this by making three key changes to the original \texttt{BERT}'s architecture. First, they factorize the large vocabulary embedding matrix used in \texttt{BERT} into two smaller ones such that dependency on the size of hidden layers is obliviated from the size of vocabulary embeddings. Second, they apply cross-layer parameter sharing. This way, the parameters are shared for similar sub-segments, thus ensuring that parameters are learned only once and are then reused for the subsequent blocks. This significantly reduces the number of trainable parameters in the model. Lastly, they propose a new inter-sentence coherence task called Sentence Order Prediction, instead of using original \texttt{BERT}'s Next Sentence Prediction (NSP). NSP is a binary classification loss that was specifically created to improve performance on downstream NLP tasks. In summary,  the \texttt{ALBERT} model is found to have 18x fewer parameters than \texttt{BERT-large} and trains 1.7x faster while achieving the state of the art results on many downstream tasks. This model is an important breakthrough as it brings the capabilities of \texttt{BERT} to a more practical and usable form that can be useful for real-world applications.      

% \subsection{Intrinsic Evaluation}
% To evaluate the quality of the embedding model, two primary methods are proposed in literature: (1) Intrinsic evaluation (2) Extrinsic evaluation.  Intrinsic evaluation refers to the class of methods to measure the quality of vector space without evaluating them on downstream tasks. For example, semantic similarity is the most traditional method to evaluate meaning representations intrinsically. 
% On the other hand, extrinsic evaluation refers to the class of methods to assess the quality of vector representation when fed as an input to the machine learning-based model in the downstream NLP task. The wide range of NLP tasks that deals with lexical semantics such as chunking, part of speech tagging,  semantic role labeling and named entity recognition can be used for the extrinsic evaluation. In this work, we restrict our study to intrinsic tasks.  
% % An important shortcoming of intrinsic evaluation is that the word similarity task measures \textit{attributional} similarity between the words. However, different NLP tasks may demand different similarity notions that need not sync with \textit{attributional} similarity. Many studies have pointed out that intrinsic evaluation is not always directly correlated with the downstream NLP application performance.
% Intrinsic evaluation directly checks for syntactic and semantic properties of words \cite{mikolov2013distributed,baroni-etal-2014-dont}. These tasks rely on query inventory datasets consisting of a query word and semantically related target word. These query inventories are readily available for resource-rich languages but not for Sanskrit. We create such inventories for four different intrinsic tasks: relatedness, synonym detection, analogy prediction, and concept categorization. For creating such query inventory dataset for these intrinsic evaluation tasks, we use \textit{Amarako\d{s}a}\footnote{\url{https://sanskrit.uohyd.ac.in/scl/amarakosha/index.html}} \cite{inproceedings_nair}, Sanskrit WordNet\footnote{\url{https://www.cfilt.iitb.ac.in/wordnet/webswn/index.php}} \cite{Kulkarni2017} and Sanskrit Heritage Reader\footnote{\url{https://sanskrit.inria.fr/DICO/reader.fr.html}} \cite{goyaldesign16,heut_13}. In extrinsic evaluation, feature extracted by word embeddings is fed as an input to downstream NLP task and corresponding performance metric is used as an indicator to compare across different embedding approaches. 
% % There is an implicit assumption that universal ranking of word embedding quality and high ranking embedding will enhance the downstream task performance. 
% Although this family of evaluation methods gives signal on the relative strength of different word embedding approaches, it needs not be considered a general proxy for overall quality.

%    \noindent\textbf{Relatedness: }
%   It is essential to distinguish between the notion of relatedness and synonyms \cite{agirre-etal-2009-study}. Synonym words share many semantic properties and they can be substituted with each other without changing the meaning of the sentences. On the other hand, semantically related words can co-occur in the same context or document and share any one semantic relationship such as meronymy or antonymy. Unlike synonym words, we can not substitute related words in place of each other. The notion of semantic relatedness between word pairs is one of the fascinating concepts in lexical semantics with a variety of NLP applications \cite{pilehvar2020embeddings}. This task is considered as an in-vitro evaluation framework for judging the quality of word embeddings.
%   The word pairs are annotated based on the degree of relatedness on a numerical scale by human annotators for evaluating semantic relatedness. For example, the distance between the \textit{paric\={a}rik\={a}} and \textit{vaidya} in the numerical scale from 0 to 3 could be 2.5 because both words belong often found together. Similarly, the human judgment score for word pair \textit{pr\={a}dhy\={a}paka - karkaṭī} could be 0.5 because these two words do not share any semantic property.
%   The word embedding performance is then evaluated by assessing the correlation between the average scores assigned by annotators and the cosine similarities between corresponding vector representations. 
  
%   For the construction of such human-annotated test data for the new target language, a standard methodology is followed in the literature \cite{camacho-collados-etal-2015-framework}. It is divided into two steps: (1) English word pairs of a standard English dataset are translated into the target language (2)  language experts annotate these word pairs. For the English language, the dataset popularized by \newcite[WordSim353]{hassan_semantic} has 353 word pairs with a human relatedness score. However, this dataset is criticized due to the human judgment criterion, which conflates similarity and relatedness. Another alternative is RG-65 \cite{RG_65} dataset. In addition, we find that many words such as \textit{automobile, cushion, autograph etc.} can not be naturally translated into Sanskrit. Therefore, we use \textit{Amarako\d{s}a} to get word pairs due to its systematic organization of semantically related words. Here,  synonymous words are categorized into synsets and semantically related words into \textit{varga}. Therefore, we decide to select the word pairs from \textit{Amarako\d{s}a}. This choice obliviates the need for translation and annotation of word pairs into Sanskrit. We exploit systematic categorization based on relatedness presents in the \textit{Amarako\d{s}a}. We transform the relatedness task into a classification task where the task is to categorize word pairs into three classes based on cosine similarity scores between vector representations generated by corresponding embeddings. For selecting word pairs, we follow the following procedure. First, we sample 13,500 word pairs in such a way that an equal proportion of word pairs are selected from the following classes : (1) word pairs from the same synset (2) word pairs from same \textit{varga} but not from the same synset (3) and the remaining word pairs such that each word from a word pair belongs to different \textit{varga}.
% %   This decision helps us to extract all possible samples to represent 0 to 3 scale uniformly. 
% %   We consider following decisions for automatic scoring. (1) The word pairs from the same synsets are marked with highest label 3. (2) word pair from the same \textit{varga} but not from same synset are marked with medium label 2 (3) a word pair belongs to different \textit{varga} is marked with the lowest label 1.
%   Out of 13,500, we use 4,500 word pairs as the development and remaining word pairs in the test set.  We use a development set to find out cosine similarity thresholds to classify word pairs into respective classes. Here, we use the macro F-score as an evaluation metric to measure the performance.
% %   With the help of annotators who are fluent speaker of Sanskrit, we collect the scores of individual annotators and the final averaging leads to final gold standard score. While annotating, we emphasized on the difference between similarity and relatedness.
  	 		 		 		 	
%  \noindent\textbf{Synonym Detection:} 
%  Synonym detection \cite{baroni-etal-2014-dont,bakarov2018survey} is a task where the goal is to find the synonym of a given target word from the four synonym candidates. In this multiple-choice setting, a single answer is correct. For example, for target \textit{sūrya\d{h}}, synonym candidates are \textit{\={a}ditya\d{h}} (correct), \textit{cañcal\={a}}, \textit{candra\d{h}} and \textit{\={a}k\={a}śa}.  Here, we choose an option as a correct answer which shows the highest cosine similarity with the target word. We use accuracy as a metric to measure performance. We leverage \textit{Amarako\d{s}a} \cite{inproceedings_nair} synsets to build MCQs. It has 4,056 synsets categorized into 25 \textit{vargas}. Out of 4,056, only 2,581 synsets have more than one element. We choose a word pair from each such synset, assign one word as the target word and another word as the correct answer. Then, for the remaining options, we use three words from the same \textit{varga} but not from the synset where the target word belongs. The primary motivation of such a choice is that words belonging to the same \textit{varga} are semantically related and picking such related words as synonym candidates make the task more interesting and challenging. Our test data has  3,034 MCQs. We consider accuracy as an evaluation metric for this task.
% %  Based of frequency of target words in training corpus, we categorized question into three categories, namely, frequently occurring, rarely occurring and not occurring. This categorization will give us proxy to infer the quality of learned representations.
 
%  \noindent\textbf{Analogy Prediction: } 
% %   There are various possible dimensions for similarity between words. For example, the notion of similarity between word pair \textit{kapi - kapibhy\={a}m} is the same as that between word pair \textit{yati - yatibhy\={a}m}. One more variant of such similarity can be word pairs \textit{prī - aprī\d{n}\={a}\d{h}} and \textit{vṛ - avṛ\d{n}\={a}\d{h}}. 
%   The analogy prediction task popularized by \newcite{mikolov2013distributed}, a question is framed with word pairs exhibiting similar sense. For example, \say{If \textit{kapi} is similar to \textit{kapibhy\={a}m} then in the same sense \textit{yati} is similar to \textit{...}}
%  Authors propose that a simple algebraic operations suffice to answer these analogy questions. In above example, in order to find similar word for \textit{yati}, we need to calculate \textit{X = vector(kapibhy\={a}m) $-$vector(kapi) +
% vector(yati)}. Then, we find the nearest neighbour to X as per cosine similarity metric and use it as answer to question.
% % Note that we do not use input words while calculating nearest neighbour.
% % Formally, this can be expressed as follows:
% %   \[X = argmax_{i} \frac{(W_{b}-W_{a}+W_{c})^T W_{i}}{||W_{b}-W_{a}+W_{c}||}\]
% %   Here , $W_{a}$, $ W_{b} \:and\: W_{c}$ refer to the word vectors of the words $a,b\: and\: c$ respectively. 
%  \begin{table}[h]
 
% \centering
% \begin{tabular}{ccccc}
% \cmidrule(r){1-5}
%  Relationship&\multicolumn{2}{c}{Word Pair 1}
% &
% \multicolumn{2}{c}{Word Pair 2} \\
% \hline
% declension&kapi& kapaya\d{h}& yati& yataya\d{h}     \\
% conjugation&ci& acīyeth\={a}m& aś& \={a}śyeth\={a}m     \\
% absolutive& dr & dīrtv\={a} & aś & aśitv\={a}      \\
% infinitive&dr& daritum & aś & aśitum     \\
% \hline
% husband - wife&vi\d{s}\d{n}u\d{h}& lak\d{s}mī& r\={a}ma\d{h}& sīt\={a}     \\
% son - father& r\={a}ma& daśaratha& abhimanyu& arjuna\\
% daughter - father&p\={a}rvatī& himav\={a}n& sīt\={a}& janaka\\
% charioteer - warrior&d\={a}ruka& kṛ\d{s}\d{n}a&  śalya& kar\d{n}a\\
% defeated - victorious&kicaka& bhīma& r\={a}va\d{n}a& r\={a}ma\\
% son - mother&kṛ\d{s}\d{n}a\d{h}&yaśod\={a}&r\={a}ma\d{h}&kauśaly\={a}\\
% \hline
% \end{tabular}
%     % \caption{Results on Sanskrit dependency parsing. Oracle MI is not comparable and is considered as upper bound for our models.}
%     \caption{Examples of syntactic (top) and semantic (bottom) questions in our test set}
%      \label{table:analogy_examples}

% \end{table}
  
%    To probe the information encoded in word embeddings, we build a comprehensive set of syntactic and semantic questions as illustrated in Table \ref{table:analogy_examples}. We use the Sanskrit Heritage Reader \cite{goyaldesign16,heut_13} for generating syntactic questions.  We consider the primary conjugation table for verbal root words and the declension table for nominal words for syntactic analogies. For conjugations, there are 10 families and popularly also called as \textit{ga\d{n}as}. Each \textit{ga\d{n}a} is further divided into \textit{parasmaipadī} and \textit{\={a}tmanepadī}. Out of these 20 families, we choose 3 representative candidates to generate primary conjugations such that most of the inflectional variations are covered. Similarly,  nominal words are broadly divided into \textit{ajanta} and \textit{halanta}. Further, they are divided based on gender and the end of root words (for example, \textit{ak\={a}r\={a}nta, uk\={a}r\={a}nta, nak\={a}r\={a}nta, jak\={a}ranta etc}). In this way, we consider 25 fine-grained families for nominals.  From each family, we select 3 representative words. Words occurring in same family display similar inflections variations. Therefore, to make questions, we strictly choose word pairs from the same family where the inflectional component belongs to the same position in the conjugation/declension table.
%   For semantic questions,  we extract semantic relation from  \textit{Amarako\d{s}a} \cite{inproceedings_nair}, \textit{R\={a}m\={a}yanam} and \textit{Mah\={a}bh\={a}ratam}.\footnote{We extract word pairs holding specific relation from wikipedia.} In semantic relationships, we consider six categories: husband - wife, son - father, daughter - father, charioteer - warrior, defeated - victorious, and son - mother. There are 6,415 semantic and 10,000 syntactic questions.  We only consider single token words in our test set.  We use accuracy as a metric to measure the performance. We evaluate accuracy separately for semantic and syntactic questions.  
% %   For semantic analogies, we depart from original evaluation setting proposed by \newcite{mikolov2013distributed}. Additionally, we also consider the synonym of actual answer as a correct answer. For example, if we consider husband - wife relation, there are more than 20 synonyms for word \textit{p\={a}rvatī} then it is too much to expect that algebraic operation returns specifically chosen word from synset as a correct answer.
  
  
%   \noindent\textbf{Categorization:}
%   As the name suggests, categorization is an evaluation task where the goal is to group nominal sets of concepts into natural categories \cite{baroni-etal-2014-dont}. For example, \textit{narmad\={a}, god\={a}varī, k\={a}verī} and \textit{gaṅg\={a}} fall under the names of river category. This task is treated as an unsupervised clustering task where word representations are clustered into \textit{n} clusters (\textit{n} is the total number of gold standard categories). Here, performance is evaluated in terms of \textit{purity}. This metric represents the degree to which elements from the single gold standard category belong to the same cluster. If unsupervised clustering exactly replicates the gold standard clusters, then the purity score reaches $100\%$. Otherwise, it decreases based on the inability to replicate gold standard partitions. 
  
%   Following \newcite{baroni-lenci-2010-distributional}, we construct a test set of 15 common categories picked from \textit{Amarako\d{s}a}. We exploit the ontological classification of \textit{Amarako\d{s}a} based on \textit{Vaiśe\d{s}ika}  ontology. 
%  \textit{Amarako\d{s}a} is also marked with semantic relations  between words. These relations are mainly classified into hierarchical and associative. We use hierarchical relations such as hypernymy - hyponymy and holonymy - meronymy for this task.
%   In each category, we select up to 10 concepts. Our categorization data contains the following categories: \textit{v\={a}dyopakara\d{n}am, vṛtti\d{h}, graha\d{h}, devat\={a}, paśu\d{h}, pak\d{s}ī, nadī, vṛk\d{s}a\d{h}, upakara\d{n}am, \={a}bhara\d{n}am, alaukikasth\={a}nam, v\={a}hanam, parvata\d{h}, vṛk\d{s}aphalam} and \textit{pu\d{s}pam}. We also build a separate test set consisting of 45 syntactic categories where each category is made up of 25 concepts.\footnote{More details can be found at: \url{https://github.com/jivnesh/EvalSan} } Each category represents a particular morphological class. 
% %   We leverage \textit{Amarako\d{s}a} to obtain y concepts from x semantic categories. We also prepare syntactic categories where y inflections from x categories are employed. 
 
% % \subsection{Extrinsic evaluation}
% % \noindent\textbf{Part of speech tagging:}  For this task, we use the recently proposed neural sequence labeling framework \cite{yang2018design}. While traditional Hidden Markov Models (HMM) and Conditional Random Fields (CRF) \cite{} based sequence labeling approaches rely on handcrafted feature engineering, with advances in deep learning, neural sequence labeling model supersedes all peers. rely on word embedding features. Model takes input as word embedding features, generate contextual representation with the help of LSTM architecture in end-to-end training and relies on CRF layer for capture label dependencies.   We presume that this task will serve as proxy for syntactic information present in word representation.
% % \begin{table}[H]
% % \centering
% % \resizebox{0.8\textwidth}{!}{%
% % \begin{tabular}{|l|l|l|l|}
% % \hline
% % \textbf{Models}  & \textbf{POS Tagging} & \textbf{Parsing}  &\textbf{Compound Identification} \\ \hline
% % Word2Vec& & & \\\hline
% % GloVe& & &  \\\hline
% % FastText & && \\\hline
% % Charagram & &&  \\\hline
% % CharLM & &&  \\\hline \hline
% % ELMo & &&  \\\hline
% % Flair & &&  \\\hline
% % BERT & &&  \\\hline \hline
% % Deepwalk & &&  \\\hline
% % Node2Vec & &&  \\\hline
% % \end{tabular}%
% % }
% % \caption{Evaluation on extrinsic tasks}
% % \label{tab:POS tagging}
% % \end{table} 

% % \noindent\textbf{Dependency Parsing:} For this task, we use a graph-based neural dependency parsing model \cite{DBLP:conf/iclr/DozatM17} similar to \newcite{kiperwasser-goldberg-2016-simple}. Neural dependency parsing model not only simplify parsing architecture but also obliviates the need of hand feature engineering. These models solely depend on word embedding based features and hence we expect that this task can be seen as proxy for both syntactic and semantic information present in word representation. In order to get contextual information of surrounding words present in a sentence, model rely on BiLSTM layers. Then, these BiLSTM extracted features are passed to MLP as a feature reduction module. Model uses biaffine attention instead of using a traditional MLP-based attention mechanism. For input vector $\vec{h}$, the affine classifier is expressed as $W\vec{h}+b$, while the biaffine classifier is expressed as $W'(W\vec{h}+b)+b'$. The choice of biaffine classifier facilitates the key benefit of representing the prior probability of word $j$ to be head and the likelihood of word $i$ getting word $j$ as the head. In this system, during training, each modifier in the predicted tree has the highest-scoring word as the head. This predicted tree need not be valid. However, at test time, to generate a valid tree MST algorithm~\cite{edmonds1967optimum} is used on the arc scores.

% % \noindent\textbf{Compound type identification:} For this task, we use a neural based automated approach for semantic class identification of compounds in Sanskrit \cite{sandhan-etal-2019-revisiting}. Here, authors demonstrate that neural approaches without any explicit feature engineering are competitive compared to traditional hand engineered feature approaches for semantic level multi-class compound classification task for Sanskrit. Contrary to previous approaches, \newcite{sandhan-etal-2019-revisiting} do not rely on hand feature engineering and only uses word embedding representation. Hence, we choose this model to evaluate the degree of semantic information present in word embedding representation. While \newcite{sandhan-etal-2019-revisiting} report results for different neural architectures and input setting, we only consider best performing configuration for our experiments.



% \subsubsection{Experiments}
% \label{experiments}
% \noindent\textbf{Corpus:}
% Our corpus contains texts from the Digital Corpus of Sanskrit (DCS), scraped data from Wikipedia and Vedabase corpus.\footnote{We use SLP1 transliteration scheme for training all the models.} The number of words in each section is 3.8 M, 1.7 M, and 0.2 M, respectively. DCS and Vedabase are segmented, but the Wikipedia data is unsegmented. We use this data for training all the embedding models. Most of the data in our corpus is in the form of poetry.

% \noindent\textbf{Hyper-parameters:} For tackling OOV problem faced by token-based embedding models such as \texttt{word2vec} and \texttt{GloVe}, we leverage \texttt{sentencepiece} tokenizer with 32,000 vocabulary size. We train \texttt{word2vec} and \texttt{GloVe} on \texttt{sentencepiece} segmented corpus. We employ following hyper-parameter settings for \texttt{word2vec} and \texttt{GloVe} : the embedding dimension size of 300, window size as 11, minimum word count for vocabulary as 1 and the number of epochs equal to 80. We keep all the remaining parameters same as used by original authors of the respective works. Next, we use raw sentences (instead of using  \texttt{sentencepiece} tokenized data) for training \texttt{FastText} and \texttt{CharLM}. We use following hyper-parameter setting for \texttt{FastText} : the embedding dimension of 300, window size of 11, the number of epochs 80, the minimum count for deciding vocabulary equals to 6, negative sampling loss with 5 negative samples, the learning rate as 0.025, minimum length of n-grams as 3 and maximum length of n-grams as 11. For \texttt{CharLM}, we use default parameters of small model architecture as \newcite{kim_charLM}.\footnote{\url{https://s3.amazonaws.com/models.huggingface.co/bert/albert-base-v2-config.json}} For \texttt{ELMo}, we use hyper-parameter settings of small model architecture.\footnote{\url{https://s3-us-west-2.amazonaws.com/allennlp/models/elmo/2x1024_128_2048cnn_1xhighway/elmo_2x1024_128_2048cnn_1xhighway_options.json}} For \texttt{ALBERT}, we use the same hyper-parameters as \texttt{albert-base-V2} model architecture except vocabulary size of 32,000 and the number of hidden layers equal to 6.


% \noindent\textbf{Results:} Table \ref{table:intrinsic_results} reports results on all the intrinsic tasks. We evaluate contextual models without context to assess how effective they are when compared with static models. Applying \textit{contextualized} models without context is similar to just using their underlying static word representation. \texttt{ELMo} outperforms all the models in all the intrinsic tasks with a large margin except the semantic categorization task. Surprisingly, with limited training data, the contextualized \texttt{ELMo} model achieved impressive overall performance compared to static models across all intrinsic tasks. The subword level segmentation with the \texttt{sentencepiece} model empowered the \texttt{word2vec} and \texttt{GloVe} to such an extent that they outperform \texttt{FastText} in analogy prediction tasks and on par in the remaining tasks. For resource-rich languages, \texttt{ALBERT} have shown the state of the art performance on many evaluation tasks. However, despite a thorough hyper-parameter search, the performance of \texttt{ALBERT} could not compete with static models. This may be due to a lack of massive training data. Similarly, except relatedness and syntactic categorization, \texttt{CharLM} model shows low performance with a large margin. 
% \begin{table}[bht]
% \begin{small}
%     \centering
% \resizebox{0.8\textwidth}{!}{%
%  \begin{tabular}{ccccccccccc|ccc}
% \toprule
%  &\multicolumn{1}{c}{Relatedness} &\multicolumn{2}{c}{Categorization} &\multicolumn{1}{c}{Similarity} &\multicolumn{2}{c}{Analogy}\\
%  \cmidrule(r){2-2}\cmidrule(l){3-4}\cmidrule(l){5-5}\cmidrule(l){6-7}
% Model &f-score&syn    & sem &acc   & syn &sem  \\
%  \cmidrule(r){2-2}\cmidrule(l){3-4}\cmidrule(l){5-5}\cmidrule(l){6-7}
% word2vec & 30.90  & 0.22 & 0.41 & 37.34 & 30.65 & 11.01 \\
% GloVe    & 31.50  & 0.25 & 0.39 & 37.41 & 30.04 & 14.01 \\
% FastText & 31.20  & 0.14 & \textbf{0.47} & 37.87 & 16.65 & 6.01  \\
% CharLM   & 35.21 & 0.33 & 0.28 & 35.94 & 2.11  & 0.03  \\
% ELMo     & \textbf{37.17} & \textbf{0.86} & 0.41 & \textbf{42.15} & \textbf{56.80}  & \textbf{32.70}  \\
% ALBERT   & 33.00    & 0.27 & 0.34 & 32.70  & 25.86 & 0.10 \\
% \toprule
% \end{tabular}}
%     \caption{Results on intrinsic evaluation tasks. For similarity and analogy prediction tasks, we use accuracy (acc) in terms of percentage as the evaluation metric, purity for categorization and f-score for the relatedness task. The syntactic and semantic tasks are denoted by \textit{syn} and \textit{sem} keywords, respectively.}
%     \label{table:intrinsic_results}
%     \end{small}
% \end{table}
% \subsubsection{Analysis}
% \noindent\textbf{Error Analysis}
% We conduct a detailed analysis of prominent mistakes done by the word embedding models. For the analogy prediction task, we find that all the models fail to correctly predict analogy questions where the root word gets modified while adding the affix to the root word. For example, in this analogy question (\textit{lip : lepsy\={a}mahe :: gur : \underline{gori\d{s}y\={a}mahe}}) while adding \textit{sy\={a}mahe} the root gets modified. On the other hand, all the models perform surprisingly well for analogy questions where affix is added without modifying root word (\textit{śak : śaknutam :: dagh : \underline{daghnutam}}). In the incorrect answers of the subword enriched \texttt{FastText} model, at least the root word is predicted correctly. \texttt{CharLM} performs the worst among all models and the predictions made by the model seem almost random with no relation to the root word or the suffix. \texttt{CharLM} learns a character level composition function to generate word-level representation. Therefore, it often predicts the correct root with an incorrect suffix or no suffix. While in the case of syntactic analogy prediction task, the \texttt{GloVe} and \texttt{word2vec} perform comparably. However, the improved performance of \texttt{GloVe} at semantic analogy task can be attributed to consideration of the global statistics of word occurrences. We observe that all the embedding models majorly get those test cases correct for similarity and relatedness tasks, which have words already present in the model vocabulary. This indicates that these models are only capable of generating representation for OOV words based on orthographic similarity and fail to capture semantic meanings. Specifically, around 55\% words present in the relatedness test set are OOV words.\footnote{Here, OOV referred as words which are not seen during training of embedding model.}  

% \noindent\textbf{Qualitative inspection for rare word}
% \label{nearest_neighbour_analysis}
%  \begin{table}[!h]
%   \begin{adjustbox}{max width=\textwidth}
% \centering
% \begin{tabular}{ccccccc}
% \cmidrule(r){1-7}
%  &\multicolumn{3}{c}{\textbf{Vocabulary words}} & \multicolumn{3}{c}{\textbf{OOV words}}\\\cmidrule(r){2-4}\cmidrule(l){5-7}
%          & \textit{nityam}      & \textit{sukham}        & \textit{t\={a}bhy\={a}m}       & \textit{ahham}      & \textit{bahūhuni}      & \textit{sahasra-cak\d{s}o}     \\
%          \cmidrule(r){2-4}\cmidrule(l){5-7} 
         
%          & nityam-eva  & sukhamayaṃ    & \={a}v\={a}bhy\={a}m      & all\={a}h      & m\={a}nini        & pracak\d{s}va         \\
% word2vec  & nityamiti   & du\d{h}kham       & dv\={a}bhy\={a}m      & ahne       & sani          & supar\d{n}\={a}\d{h}-ca       \\
%          & sad\={a}        & sukha-du\d{h}kham & tay\={a}          & ahrasat    & cūr\d{n}it\={a}ni     & pracak\d{s}mahe       \\
%           \cmidrule(r){2-4}\cmidrule(l){5-7} 
%          & nityamiti   & sukhamayaṃ    & adhik\={a}ribhy\={a}m & all\={a}h      & bahū          & tat-ca-eva        \\
% GloVe    & nityam-eva  & du\d{h}kham       & p\={a}r\d{s}\d{n}ibhy\={a}m   & ahne       & behul\={a}        & tath\={a}-ca          \\
%          & sad\={a}        & du\d{h}khameva    & jaṅgh\={a}bhy\={a}m   & ahnuvi     & behul\={a}y\={a}\d{h}     & yat-ca-eva        \\
%           \cmidrule(r){2-4}\cmidrule(l){5-7} 
%          & sad\={a}        & su-sukham     & tayo\d{h}         & simham     & bahuni        & sahasraḷaṃ\d{n}tra    \\
% FastText & satatam     & du\d{h}kham       & tau           & tam        & mandmatyo\d{h}    & sahasra-kṛtvas    \\
%          & nitya-sn\={a}yī & sukha-du\d{h}kham & cak\d{s}uḍbhy\={a}m   & yath\={a}-aham & bahava\d{h}-tatra & sahasra-vedhī     \\
%           \cmidrule(r){2-4}\cmidrule(l){5-7} 
%          & sṭeḍiyam    & somam         & sabh\={a}y\={a}\d{h}      & īḍyam      & vatsyati      & paryaṭanasthale\d{s}u \\
% CharLM   & samśayam    & saudham       & ny\={a}yasabh\={a}y\={a}\d{h} & bṛhantam   & yotsyati      & na\d{s}ṭa-saṃjña\d{h}     \\
%          & y\={a}payan     & homam         & hast\={a}bhy\={a}m    & gayam      & setsyati      & c\={a}k\d{s}u\d{s}asya-antare \\
%           \cmidrule(r){2-4}\cmidrule(l){5-7} 
%          & martyam     & sakham        & n\={a}bhy\={a}m       & arham      & vil\={a}sini      & aj\={a}ta-śatro       \\
% ELMO     & ni\d{s}ṭham     & kulam         & y\={a}bhy\={a}m       & aṅkam      & mattak\={a}śini   & sahasra-śīr\d{s}\={a}     \\
%          & yugyam      & sukh\={a}m        & bhūbhy\={a}m      & andham     & j\={a}nuni        & ahu-rūpa\d{h}         \\
%           \cmidrule(r){2-4}\cmidrule(l){5-7} 
%          & d\={a}nam       & sat\={a}m         & ardham        & ahrasam    & ityadīni      & ūrdhva-ge         \\
% ALBERT   & loke        & padam         & mandam        & all\={a}h      & hras\={a}ni       & sahasra-śīr\d{s}\={a}     \\
%          & bhavit\={a}     & k\d{s}ayam        & dhairyam      & ahnuth\={a}\d{h}   & maṃdiram      & sarva-mahīk\d{s}it\={a}m  \\
% \hline
% \end{tabular}
%    \end{adjustbox}
%     % \caption{Results on Sanskrit dependency parsing. Oracle MI is not comparable and is considered as upper bound for our models.}
%     \caption{Nearest neighbours (based on cosine similarity) for in vocabulary and  OOV words for the models trained on Sanskrit corpus. Last three words are OOV words. We use contextual models without a context. Applying \textit{contextualized} models without context is very similar to just using their underlying static word representation.}
%      \label{table:in_vs_out_vocab}
  
 
% \end{table}
% We analyze the word representations captured by different models. We consider \textit{contextualized} models also in this experiment. We use contextual models without a context to assess how effective are they when compared with static models. Applying \textit{contextualized} models without context is very similar to just using their underlying static word representation. For systematic investigation, we choose three representative words from following categories: (1) In Vocabulary words (2) Out of Vocabulary words. Table \ref{table:in_vs_out_vocab} illustrates the top three nearest neighbors based on cosine similarity between embeddings learned by different models. For frequently occurring words present in vocabulary all the embeddings except \texttt{CharLM} and \texttt{ALBERT} are able to capture lexical meaning. The quality of nearest neighbour candidates of \texttt{CharLM} and \texttt{ALBERT} is relatively poor compared to other models. We suspect that the possible reason for this behaviour may be due to less amount of training data.  The subword level modeling in \texttt{word2vec}, \texttt{GloVe} and \texttt{FastText} makes these models more inclined to find words which are orthographically similar. For these models, the representations seems to depend on surface string. For example, the nearest neighbours of \textit{nityam} and \textit{sukham} are very close in terms of edit distance. On the other hand, \texttt{ELMo} not only captures semantic level features but also orthographic features. This is very well evident from the following examples. The nearest neighbours produced by \texttt{ELMo} for \textit{nityam} and \textit{sukham} are lexically similar but orthographically different in terms of edit distance. However, the nearest neighbours of \textit{t\={a}bhy\={a}m} exhibits suffix similarity. The last three words are OOV where \textit{ahham}, \textit{bahūhuni} are words with incorrect spelling and \textit{sahasra-cak\d{s}o} is the compound word. For OOV words also  similar trend holds. We generate representation for OOV for \texttt{word2vec} and \texttt{GloVe} using \texttt{sentencepiece} tokenizer. This tokenizer breaks OOV into subwords available in \texttt{sentencepiece} model vocabulary and representation of OOV word is sum of representations of these segmented subwords. 



% \noindent\textbf{Qualitative inspection of contextualized embeddings}
% \label{context_cluster}
% \begin{figure}[!h]
% \centering
% \subfigure[]{\includegraphics[width=2.5in]{images/chakri_elmo.png}} 
% \subfigure[]{\includegraphics[width=2.5in]{images/chakri_ALBERT.png}}\\
% \caption{Projection of contextualized representation (the left side : \texttt{ELMo} and the right side \texttt{ALBERT}) for different sense of polysemous word \textit{cakrī} denoted by following sentences: \textit{(1) cakrī mṛd\={a} jalena ca kumbhanirm\={a}\d{n}e viś\={a}rada\d{h}
% (2) cakrī kevala jala mṛd cakra upajīvaka\d{h}
% (3) cakrī cakrasya upari mṛda\d{h} kumbhaṃ nirm\={a}ti
% (4) svahaste bibharti sudarśanam sa cakrī
% (5) sudarśanena cakrī śiśup\={a}lam jagh\={a}na
% (6) rak\d{s}obhya\d{h} svabhakt\={a}n tr\={a}tum cakrī sudarśanam bibharti.}} 
% \label{fig:chakri} 
% \end{figure}
% \begin{figure}[!h]
% \centering
% \subfigure[]{\includegraphics[width=2.5in]{images/hari_elmo.png}} 
% \subfigure[]{\includegraphics[width=2.5in]{images/chakri_ALBERT.png}}\\
% \caption{Projection of contextualized representation (the left side : \texttt{ELMo} and the right side \texttt{ALBERT}) for different sense of polysemous word \textit{hari\d{h}} denoted by following sentences: \textit{(1) v\={a}yusuta\d{h} hari\d{h} v\={a}nar\={a}\d{n}\={a}m to\d{s}am vavardha
% (2) sugrīva\d{h} n\={a}ma hari\d{h} v\={a}nar\={a}\d{n}\={a}m r\={a}j\={a} \={a}sīt
% (3) v\={a}nar\={a}\d{n}\={a}m vṛddha\d{h} hari\d{h} j\={a}mbav\={a}n
% (4) hari\d{h} bale\d{h} trailokyasampadam chalena jah\={a}ra
% (5) hari\d{h} hira\d{n}y\={a}k\d{s}am nihatya devat\={a}n\={a}m khedam jah\={a}ra
% (6) hari\d{h} rukmi\d{n}īm jah\={a}ra paśyat\={a}m}} 
% \label{fig:harih} 
% \end{figure}
% To investigate the contextualized nature of \texttt{ELMo} and \texttt{ALBERT}, we analyze the vector representation (using PCA to project the vectors into 2D space) of a two polysemous words in different context. In this experiment, each test case consists of 6 sentences in Sanskrit such that all sentences have one common polysemous word. Out of 6 sentences, 3 sentences represent one sense of meaning and the remaining represent another sense of meaning for that common polysemous word. Ideally, contextualized word vectors representing the same sense of meaning should form a cluster. For the polysemous word \textit{cakrī}, we consider two senses of meaning, namely, potter and the Lord Vi\d{s}\d{n}u. This test set consists of 6 sentences as follows: \textit{(1) cakrī mṛd\={a} jalena ca kumbhanirm\={a}\d{n}e viś\={a}rada\d{h}
% (2) cakrī kevala-jala-mṛd-cakra-upajīvaka\d{h}
% (3) cakrī cakrasya upari mṛda\d{h} kumbhaṃ nirm\={a}ti
% (4) svahaste bibharti sudarśanam sa cakrī
% (5) sudarśanena cakrī śiśup\={a}lam jagh\={a}na
% (6) rak\d{s}obhya\d{h} svabhakt\={a}n tr\={a}tum cakrī sudarśanam bibharti.} For the first three sentences, the sense of the meaning of the word \textit{cakrī} is a potter and for the remaining sentences, the sense of meaning is the Lord Vi\d{s}\d{n}u.  Figure \ref{fig:chakri} illustrates visualization of polysemous word \textit{cakrī}. Here, we observe that the contextualized representation indicating the same sense of meaning are clustered together. Similarly, we consider another polysemous word \textit{hari\d{h}} consists of two senses of meaning, namely, monkey and the Lord Vi\d{s}\d{n}u. \textit{(1) v\={a}yusuta\d{h} hari\d{h} v\={a}nar\={a}\d{n}\={a}m to\d{s}am vavardha
% (2) sugrīva\d{h} n\={a}ma hari\d{h} v\={a}nar\={a}\d{n}\={a}m r\={a}j\={a} \={a}sīt
% (3) v\={a}nar\={a}\d{n}\={a}m vṛddha\d{h} hari\d{h} j\={a}mbav\={a}n
% (4) hari\d{h} bale\d{h} trailokyasampadam chalena jah\={a}ra
% (5) hari\d{h} hira\d{n}y\={a}k\d{s}am nihatya devat\={a}n\={a}m khedam jah\={a}ra
% (6) hari\d{h} rukmi\d{n}īm jah\={a}ra paśyat\={a}m}. In Figure \ref{fig:harih}, we find the similar trend for this test case. The qualitative analysis suggests that the \textit{contextualized} representations generated by \newcite{elmo} and \newcite{ALBERT:} for polysemous words indicating the same sense of meaning forms a cluster for each sense of meaning (Section \ref{context_cluster}). 
% This is indeed a serendipitous outcome for such data-hungry models when trained on negligibly small amount of corpus available for Sanskrit.


%  \begin{table}[H]
%   \begin{small}
% \centering
% \begin{tabular}{ccc}
% \textbf{word} & \textbf{context} & \textbf{nearest neighbour} \\ \hline
% Washington & (a) Washington to curb support for [..]& (1) Washington would also take [..] action [..] \\
% & &   (2) Washington would also take [..] action [..] \\
% \hline
% Washington & (a) Washington to curb support for [..]& (1) Washington would also take [..] action [..] \\
% & &   (2) Washington would also take [..] action [..] \\
% \hline
% Washington & (a) Washington to curb support for [..]& (1) Washington would also take [..] action [..] \\
% & &   (2) Washington would also take [..] action [..] \\
% \hline
% Washington & (a) Washington to curb support for [..]& (1) Washington would also take [..] action [..] \\
% & &   (2) Washington would also take [..] action [..] \\
% \hline
% \end{tabular}
%     % \caption{Results on Sanskrit dependency parsing. Oracle MI is not comparable and is considered as upper bound for our models.}
%     \caption{Nearest neighbour in different context.}
%      \label{table:context neighbour}
%      \end{small}
% \end{table}

\section{Summary}
We present the first neural-based Sanskrit NLP toolkit, SanskritShala which facilitates diverse linguistic analysis for tasks such as word segmentation, morphological tagging, dependency parsing and compound type identification. It is set up as a web-based application to make the toolkit easier to use for teaching and annotating. All the codebase, datasets and web-based applications are publicly available. We also release word embedding models trained on publicly available Sanskrit corpora and various annotated datasets for 4 intrinsic evaluation tasks to access the intrinsic properties of word embeddings. We strongly believe that our toolkit will benefit people who are willing to work with Sanskrit and will eventually accelerate the Sanskrit NLP research.

==> List_of_Publication.tex <==
\chapter*{List of Publications}
\thispagestyle{empty}
\begin{enumerate}
    \itemhrefereed journals based on thesis
        whatever \par
    \item refereed journals (others)
        whatever \par
    \item presentations in conferences
        whatever \par
    \itemhead publications in conference proceedings
        whatever \par
\end{enumerate}
\vfill


==> acro_list.tex <==
\begin{acronym}[XXXXXXXXX] % Give the longest label here so that the list is nicely aligned
\acro{TransLIST}{Transformer-based Linguistically Informed Sanskrit Tokenizer}
\acro{SaCTI}{Sanskrit Compound Type Identification}
\acro{SCL}{Sanskrit Computational Linguistics}
\acro{NLP}{Natural Language Processing}
% \acro{SEM}{scanning electron microscope}
% \acro{WHA}{tungsten heavy alloys}
% \acro{SPS}{spark plasma sintering}
% \acro{ND}{normal direction to the rolling plane}
% \acro{CD}{compression direction}
% \acro{RD}{rolling direction in a rolled plate}
% \acro{LD}{Loading direction}
% \acro{TD}{transverse direction in a rolled plate}
% \acro{XRD}{X-ray diffraction}
% \acro{ODF}{orientation distribution function}
% \acro{OM}{optical microscope}
% \acro{IQ}{image quality}
% \acro{IPF}{inverse pole figure}
% \acro{FESEM}{field emission scanning electron microscopy}
% \acro{f.c.c.}{face centred cubic}
% \acro{b.c.c.}{body centred cubic}
% \acro{EPMA}{electron probe microanalyser}
% \acro{EDS}{energy dispersive spectrometer}
% \acro{LPS}{liquid phase sintering}
% \acro{FFT}{fast Fourier transform}
% \acro{HEM}{homogeneous effective medium}
% \acro{RVE}{representative volume element}
% \acro{CRSS}{critical resolved shear stress}
% \acro{PF}{pole figure}
% \acro{VPSC}{viscoplastic self-consistent}
% \acro{STECA}{Stress Texture Calculator}
% \acro{DAMASK}{D\"{u}sseldorf Advanced Material Simulation Kit}
% \acro{KAM}{kernal average misorientation}
% \acro{GND}{geometry necessary dislocation}
% \acro{GROD}{grain reference orientation deviation}
% \acro{CAD}{computer-aided design}
% \acro{AVACS}{average number of active systems per grain}
% \acro{SRO}{short range ordering}
% \acro{TWIP}{twinning induced plasticity}
% \acro{TRIP}{transformation induced plasticity}
% \acro{h.c.p.}{hexagonal close packed}
% \acro{YS}{yield strength}
% \acro{UTS}{ultimate tensile strength}
% \acro{MSBs}{micro-shear bands}
% \acro{DB}{deformation bands}
% \acro{TB}{transition bands}
% \acro{SFE}{stacking fault energy}
% \acro{SHPB}{split-Hopkinson pressure bar}
% \acro{ppm}{parts per million}
% \acro{CES}{Cambridge Engineering Selector}
% \acro{DBTT}{ductile-to-brittle transition temperature}
% \acro{mrd}{multiples of a random distribution}
% \acro{FWHM}{full width at half maximum}
% \acro{CPFEM}{crystal plasticity finite element methods}

\end{acronym}
